Ego-Exo: Transferring Visual Representations from Third-person to First-person Videos

We introduce an approach for pre-training egocentric video models using large-scale third-person video datasets. Learning from purely egocentric data is limited by low dataset scale and diversity, while using purely exocentric (third-person) data introduces a large domain mismatch. Our idea is to discover latent signals in third-person video that are predictive of key egocentric-specific properties. Incorporating these signals as knowledge distillation losses during pre-training results in models that benefit from both the scale and diversity of third-person video data, as well as representations that capture salient egocentric properties. Our experiments show that our Ego-Exo framework can be seamlessly integrated into standard video models; it outperforms all baselines when fine-tuned for egocentric activity recognition, achieving state-of-the-art results on Charades-Ego and EPIC-Kitchens-100.

==> Ego-Exo_CVPR21 (ArXiv)_4:14:2021/sections/abstract.tex <==
% \TN{Egocentric video presents a unique viewpoint tied to the camera wearer's intentions and activities. Though powerful for explaining human behaviour, these unique features make training egocentric video models difficult. Learning from purely egocentric data is limited by dataset scale, while using purely exocentric \KG{(third-person)} data introduces a large domain mismatch.}
We introduce an approach for pre-training \emph{egocentric} video models using large-scale \emph{third-person} video datasets. Learning from purely egocentric data is limited by low dataset scale and diversity, while using purely exocentric (third-person) data introduces a large domain mismatch. %Thus, our main idea 
Our idea is to discover latent signals in third-person video that are predictive of key egocentric-specific properties. Incorporating these signals as knowledge distillation losses during pre-training results in models that benefit from both the scale and diversity of third-person video data, as well as representations that capture salient egocentric properties. %features. 
%Our experiments on EPIC-Kitchens and Charades-Ego show that our ``Ego-Exo'' pre-trained model outperforms all baselines when fine-tuned for activity recognition, %and can be seamlessly integrated into state-of-the-art models to further boost performance. % 
Our experiments show that our ``Ego-Exo'' framework can be seamlessly integrated into standard video models; it outperforms all baselines when fine-tuned for egocentric activity recognition, achieving state-of-the-art results on Charades-Ego and EPIC-Kitchens-100.

%\KGnote{We could shorten this if needed, e.g., remove first 3 sentences.}



% pure text
% We introduce an approach for pre-training egocentric video models using large-scale third-person video datasets. Learning from purely egocentric data is limited by low dataset scale and diversity, while using purely exocentric (third-person) data introduces a large domain mismatch. Our idea is to discover latent signals in third-person video that are predictive of key egocentric-specific properties. Incorporating these signals as knowledge distillation losses during pre-training results in models that benefit from both the scale and diversity of third-person video data, as well as representations that capture salient egocentric properties. Our experiments show that our Ego-Exo framework can be seamlessly integrated into standard video models; it outperforms all baselines when fine-tuned for egocentric activity recognition, achieving state-of-the-art results on Charades-Ego and EPIC-Kitchens-100.

==> Ego-Exo_CVPR21 (ArXiv)_4:14:2021/sections/conclusion.tex <==
\section{Conclusion}
We proposed a novel method to embed key egocentric signals into the traditional third-person video pre-training pipeline, so that models could benefit from both the scale and diversity of third-person video datasets, and create strong video representations for downstream egocentric understanding tasks.
Our experiments show the viability of our approach as a drop-in replacement for the standard Kinetics-pretrained video model, achieving state-of-the-art results on egocentric action recognition on Charades-Ego and EPIC-Kitchens-100. 
Future work could explore alternate distillation tasks and instance-specific distillation losses to maximize the impact of third-person data for training egocentric video models. % and scenarios to facilitate the egocentric video understanding research.
% \TNnote{YL, fill out some future directions/applications?}


\vspace{0.1in}
\noindent\textbf{Acknowledgments}: UT Austin is supported in part by the NSF AI Institute and FB Cognitive Science Consortium.

==> Ego-Exo_CVPR21 (ArXiv)_4:14:2021/sections/exp.tex <==
\section{Experiments}~\label{sec:exp}
% \YLnote{Use pre-trained everywhere}
% \BOnote{Use distillation during pre-training and fine-tuning \cite{chen2020big}. We can just add the reference when we discuss using distillation for fine-tuning.}


% \subsection{Baselines}
\vspace{-10mm}
% \subsection{Datasets}
\paragraph{Datasets.} 
%\noindent\textbf{Datasets.}
% For the experiments, we \TN{use the following datasets}.% conduct the standard third-person video dataset Kinetics~\cite{kinetics} for pre-training, and then evaluated on three three popular egocentric datasets.
Our experiments use the following datasets.
\begin{itemize}[leftmargin=*]
\vspace{-1mm}
\setlength\itemsep{0em}
\item \textbf{Kinetics-400}~\cite{kinetics} is a popular third-person video dataset containing $\sim$300k videos %240k training videos and ~20k validation videos 
and spanning 400 human action classes. %\cc{, resulting in around 850 hours videos in total.}
We use this dataset to pre-train all our models.
%\KGnote{give simple justification for why Kinetics vs any other}
\item \textbf{Charades-Ego}~\cite{charades-ego} has $\sim$68k %\TN{video}
 % \YLnote{(they are claiming activity not video as the videos are multi-label)} 
instances spanning 157 activity classes. %recorded in 112 homes.
Each instance is a pair of videos corresponding to the same activity, recorded in the first and third-person perspective.  Our method does not require this pairing, and succeeds even if no pairs exist (Supp.). %Charades-Ego is a paired dataset in which first-person and third-person videos are paired with their counterparts. 

%---we use only the first-person videos to evaluate our models. % we evaluate methods on the 34.4 hours of first-person videos in Charades-Ego. 
% \item EGTEA [optional]
\item \textbf{EPIC-Kitchens}~\cite{epic} is an egocentric video dataset with videos of non-scripted daily activities in kitchens. It contains 55 hours of videos consisting of 39k action segments, annotated for interactions spanning 352 objects and 125 verbs. \textbf{EPIC-Kitchens-100}~\cite{epic-100} extends this to 100 hours and 90k action segments, and is currently the largest annotated egocentric video dataset. 
% \item \textbf{Epic-Kitchen-100}~\cite{epic-100} is the current largest annotated egocentric dataset which extends Epic-Kitchens~\cite{epic} to 100 hours and 90k action segments. 
\end{itemize}

Due to its large scale and diverse coverage of actions, Kinetics has widely been adopted as the standard dataset for pre-training both first- and third-person video models~\cite{gu2018ava,slowfast,epic-fusion,epic-100}. %pre-trained models are widely adopted by other datasets, including both third-person datasets~\cite{} and egocentric datasets~\cite{}. 
EPIC-Kitchens and Charades-Ego are two large and challenging egocentric video datasets that are the subject of recent benchmarks and challenges.

%\vspace{-2mm}
\paragraph{Evaluation metrics.}
%\noindent\textbf{Evaluation metrics.}
%In our experiments, 
We pre-train all models on Kinetics, and fine-tune on Charades-Ego (first-person only) and EPIC-Kitchens for activity recognition. Following standard practice, %for Charades-Ego, 
we report mean average precision (mAP) for Charades-Ego %across 157 activity classes. For EPIC-Kitchens, we report top-1 and top-5 accuracy for verbs, nouns, and actions. 
and top-1 and top-5 accuracy for EPIC. %-Kitchens.
% \YLnote{Need update if we add anticipation}

%\vspace{-2mm}
\paragraph{Implementation details.} 
%\noindent\textbf{Implementation details.}
% \TNnote{Move parts to Supp. if needed}
We build our Ego-Exo framework on top of PySlowFast~\cite{pyslowfast} and use SlowFast~\cite{slowfast} video models %from Slow-only and SlowFast~\cite{slowfast} as the video models with ResNet~\cite{resnet}
as backbones with $8$ input frames and stride $8$. %$(8 \times 8)$-ResNet50 configuration. 
We use a Slow-only ResNet50 architecture for all ablation experiments, and  a SlowFast ResNet50/101 architecture for final results. %final results. % with  frames as the input clip, where we sample $8$ frames with stride $8$. 

For our distillation heads $H^{ego}$ and $H^{obj}$ (Sec~\ref{sec:tasks}), we use a spatiotemporal pooling layer, followed by a linear classifier. We implement our Interaction-Map heads $H^{h}$ and $H^{o}$ as two 3D conv layers with kernel sizes $1{\mkern-2mu\times\mkern-2mu}3{\mkern-2mu\times\mkern-2mu}3$ and $1{\mkern-2mu\times\mkern-2mu}1{\mkern-2mu\times\mkern-2mu}1$, and ReLU activation. 

For our combined loss function (Eqn~\ref{eqn:loss})%Ego-Exo
, we set the %parameters in the auxiliary tasks through cross-validation on the validation set of Epic-Kitchen~\cite{epic}. The temperature parameter $T$ is set to 1 and 
loss weights $w_{ego}$, $w_{obj}$ and $w_{int}$ to $0.1, 0.5, 1.0$ respectively through cross-validation on the EPIC-Kitchens validation set (cross-validation on Charades-Ego suggested
similar weights).
%\TNnote{Can we say this? Or is this untrue?} \KGnote{seems good way to note it.}\YLnote{It's true but the actual experiments are conducted on the test set. Could we just say "we conduct the same weights on Charades-Ego" to be safe?} \KGnote{if it is set only once on that dataset, it conflicts with the statement above in approach that we set it by validation on each downstream task.}\YLnote{Actually, it performs similarly on both charades-ego and epic. Since charades-ego didn't have a standard validation set, I only say Epic here.}  
The temperature parameter $\beta$ in Eqn~\ref{eqn:yego} and Eqn~\ref{eqn:yobj} is set to 1. 
%\TNnote{Previously it said these weight parameters are different for each dataset? i.e. EPIC should have a different set of weights than Charades-Ego?} \YLnote{The final trend is very similar, so I am choosing the same weights for all datasets.}
% \paragraph{Pre-training and fine-tuning.} For different pre-training models, we first train the video models from scratch on Kinetics-400. Then we conduct the pre-trained video model as initialization and fine-tuning on different tasks on different egocentric tasks. See training details on different datasets in Appendix.
Training schedule and optimization details can be found in Supp.


\subsection{Ego-Exo pre-training}









We compare our pre-training strategy to these methods: 
% \paragraph{Different pre-training models.} We compare against the following methods:
\begin{itemize}[leftmargin=*]
\vspace{-1mm}
\setlength\itemsep{-0.3em} 
    \item \textbf{Scratch} does not benefit from any pre-training. It is randomly initialized and directly fine-tuned on the target egocentric dataset.
    \item \textbf{Third-only} is pre-trained for activity labels on Kinetics 400~\cite{kinetics}. This represents the status-quo pre-training strategy for current video models.
    \item \textbf{First-only} is pre-trained for verb/noun labels on EPIC-Kitchens-100~\cite{epic-100}, the largest publicly available egocentric dataset. %for pre-training.
    % Note \TN{that} we only evaluate on Charades-Ego here as EPIC-Kitchens is used for pre-training.
    \item \textbf{Domain-adapt} % uses unlabeled egocentric video
    introduces a domain adaptation loss derived from gradients of a classifier trained to distinguish between first- and third-person video instances~\cite{ganin2016domain}.
    % as target domain to adapt third-person videos from Kinetics using a domain adaptation loss~\cite{ganin2016domain}. %, which is also adapted .
    %adds a domain adaptation loss during pre-training using unlabeled egocentric video from the target dataset.
    %We propagate negative gradients~\cite{ganin2016domain} from the classifier to the video backbone %using the gradient reversal layer~\cite{ganin2016domain}
    This strategy has been used in recent work to learn domain invariant features for third-person vs.~drone footage~\cite{choi2020unsupervised}. %\TNnote{I think it's important to keep these details in. Just "domain adaptation loss" is too vague.}
    %a recent domain adaptation strategy~\cite{} to bridge the first-third person gap by utilizing unlabeled instances from the target egocentric dataset. \YLnote{TN could update it?} \KGnote{try to spell out where DA has been used for first-third person work before, and how representative this method is for them (maybe it's only one method?}
    \item \textbf{Joint-embed} uses paired first- and third-person video data from Charades-Ego to learn viewpoint-invariant video models via standard triplet embedding losses~\cite{sigurdsson2018actor}. We first pre-train this model with Kinetics to ensure that the model benefits from large-scale pre-training. 
    % Note that this baseline assumes access to paired video data, which our method does not require. \YLnote{remove to save space.}
    % \YLnote{Is that safe to cite directly as }
    % \item  \textsc{ImageNet-KD~\cite{girdhar2019distinit}} is pre-trained with third-person data, but distills knowledge from ImageNet~\cite{deng2009imagenet} labels to enhance pre-training. This baseline does not leverage any egocentric cues in the knowledge distillation process. \TNnote{Can be ablation instead of method.}
    % \item \textsc{Multi-task} adds up losses for multiple tasks across both first and third person datasets, specifically, action classification on Kinetics and gaze prediction(???) on EGTEA+ (???) as the pre-training objective. \TNnote{Need something to preempt the question: "but you're using pre-trained ego models to generate egoscore/objscore/intmap. What about the data they were trained on?"}
    \item \textbf{Ego-Exo} is pre-trained on Kinetics-400, but additionally incorporates  %We add
    the three auxiliary egocentric tasks (Sec~\ref{sec:tasks}) together with the original action classification loss, to learn egocentric-specific features during pre-training. % from Kinetics-400 to form our Ego-Exo pre-trained model.
    % \KGnote{should we mention ego-exo* at this time?} \YLnote{Right now, it's introduced in Table 3. As it needs some explanations, I feel maybe we could still keep it in the second ablation study?} TN: I agree. It can show up in the later section when we also upgrade the backbone.
\vspace{-1mm}
\end{itemize}
For this experiment, all models share the same backbone architecture (Slow-only, ResNet-50)
and only the pre-training strategy is varied to ensure fair comparisons. \emph{Domain Adapt} uses additional unlabeled egocentric data during pre-training, but from the same target dataset that the model will have access to during fine-tuning. \emph{Joint-embed} uses paired egocentric and third-person data, an advantage that the other methods do not have, but offers insight into performance in this setting.  Only \emph{First-only} has access to ego-videos labeled for actions during pre-training.  %Then we conduct

% \TN{These} different pre-trained models \TN{are then} fine-tuned on Charades-Ego and Epic-Kitchen. %datasets, respectively.
%\TNnote{Consider \textbackslash textsc for methods. ``Third-only'' $\rightarrow$ \textsc{Third-only}. Normal text appearing in the middle of the para is a little bit confusing.} \YLnote{I dont' have a strong preference here. If so, are you suggesting use textsc for all tables, including SOTA in Table 4 and 5?}
%\YLnote{Use \emph for methods}

\begin{table}[t]
\small
%\renewcommand\arraystretch{1.1}
	\begin{center}
	\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{l|c|cc|cc}
		%\hline
		    &  C-Ego & \multicolumn{2}{c|}{EPIC verbs} & \multicolumn{2}{c}{EPIC nouns} \\
		\cline{2-6}
		Methods	&  mAP  & top-1 & top-5 & top-1 & top-5	\\
		\hline
        % Scratch  & 8.37 & 46.16	& 84.24 &	26.98	& 51.83 \\
        % First-only & 11.80  & -- & -- & -- & --	  \\
        % Third-only & 24.83 &	61.34&	\textbf{87.41}&	45.95&	\textbf{70.18} \\
        % Domain-adapt~\cite{ganin2016domain} & 23.71 & 60.84 & \textbf{87.41} & 45.66 & 68.27 	  \\
        % Joint-embed~\cite{sigurdsson2018actor} & - & \YL{45.12} & \YL{83.07} & \YL{27.44} & \YL{48.67} 	  \\
        % Ego-Exo       & \textbf{26.35} & \textbf{63.34} &	87.36 &	\textbf{47.21} &	69.89 \\
        Scratch  & 8.50 & 55.62 & 86.10 & 38.35 & 62.39 \\
        First-only & 11.73  & -- & -- & -- & --	  \\
        Third-only & 24.69 & 61.19 & 87.49 & 46.18 & 69.72 \\
        Domain-adapt~\cite{ganin2016domain} & 23.62 & 61.27 & 87.49 & 45.93 & 68.73 	  \\
        Joint-embed~\cite{sigurdsson2018actor} & - & 61.26 & 87.17 & 46.55 & 68.97	  \\
        Ego-Exo       & \textbf{26.23} & \textbf{62.83} & \textbf{87.63} & \textbf{48.15} & \textbf{70.28} \\
		\hline				
	\end{tabular}
	\end{center}
\vspace{-5mm}
\caption{\textbf{Ego-Exo vs.~alternate pre-training methods.} 
%First- or third-person data alone is insufficient ---our auxiliary distillation losses results in best performance.
Our Ego-Exo pre-training results in best performance.
%\TN{Validation set} results are generated using the Slow-only model. 
Note that we do not evaluate \emph{First-only} and \emph{Joint-embed} on the datasets they were pre-trained on (EPIC and Charades-Ego respectively). Values are averaged over 3 runs. 
%\KGnote{should our num here agree with the num in table 4 for charades?}\YLnote{It's different as In Table 1-3, we use Slow-only as backbone while Table 4-5 use SlowFast. Also in this table, the compared methods are implemented by ourself using Slow-only}
% \TNnote{Updated 3-run for DA}
%\YLnote{need update 3-run for DA and Joint-embed} \TNnote{Even scratch/first-only/third-only need to be updated to 3-run?} \YLnote{yes, already updated. Main variance comes from Epic.}
%\TNnote{We could also do Charades-1st pretraining for EPIC. It'll be terrible since Charades is so small, but we won't have dashes in the table. Thoughts?} 
%\YLnote{IMO, I prefer not have that as Charades is smaller than Epic, it seems not making sense to pretrain on small dataset and fine-tune on the larger one?}
% \KGnote{add bolds when ready.}  
% should we ref ~\cite{sigurdsson2018actor} next to Joint-embed? is the implementation strictly close enough? 
% \KGnote{reader may wonder where the action col is for EPIC?}
% \YLnote{It's not a full re-implementation since we plan to implement the triplet loss which would one of two components in their method. For Table 1-3, I don't include Epic-action for simplicity. Let me know if you prefer to add it}
% }
% \TNnote{Still think it's okay to add \cite{sigurdsson2018actor}. It's the same basic idea and we'll give all details/differences in Supp. Reg action col: I think we can skip for space. I replaced Charades-Ego with Charades to make cols smaller.}
%\TNnote{Will top-5 results look any better if we report on the more popular EPIC split? (SlowFast/LFB split)}
%\YLnote{I think variance among runs matters here. Maybe having a 3-run average for all ablation studies? I also noticed the similar variance in another split}
%\YLnote{Joint-Embed may still be improved by tuning. }
% \YLnote{How about making the name `C-Ego` as Charades is an existing dataset which may cause confusion?}
}
\vspace{-1mm}
\label{tb:different_baseline}
\end{table}



\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
	\setlength{\tabcolsep}{3pt}
	\begin{tabular}{l|ccc|c|cc|cc}
		%\hline
		    & & & & C-Ego & \multicolumn{2}{c|}{EPIC verbs} & \multicolumn{2}{c}{EPIC nouns} \\
		\cline{5-9}
 		Methods	& $\tau^{ego}$ & $\tau^{obj}$ & $\tau^{h+o}$ & mAP  & top-1 & top-5 & top-1 & top-5	\\
%        Methods	& Ego-score & Object-score & Interaction-map & mAP  & top-1 & top-5 & top-1 & top-5	\\
		\hline
        Third-only & \xmark & \xmark & \xmark & 24.69 & 61.19 & 87.49 & 46.18 & 69.72\\
        \hline
        \multirow{5}{*}{Ego-Exo} & \cmark & \xmark & \xmark & 25.01 & 62.22 & 87.78 & 46.26 & 68.76 \\
            &  \xmark & \cmark & \xmark & 25.49 & 61.65 & 87.57 & 46.27 & 69.52\\
            &  \xmark & \xmark & \cmark & 25.91 & 62.55 & \textbf{88.50} & 47.71 & 69.62\\
         %   &  \cmark & \cmark & \xmark & 25.73 & 62.47	&   \textbf{88.32}	&   47.04   &	\textbf{70.35}\\
            &  \cmark & \cmark & \cmark & \textbf{26.23} & \textbf{62.83} & 87.63 & \textbf{48.15} & \textbf{70.28} 	\\
		\hline				
	\end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Auxiliary task ablation study.} Distilling knowledge from all three egocentric tasks results in the best performing pre-trained model. Values are averaged over 3 runs.
}
\vspace{-3mm}
%\TN{Validation set} results are generated using the Slow-only model.
%on Charades-Ego and Epic-Kitchen datasets with Slow-only model. 
%\YLnote{maybe worth to have multiple runs for epic-55 as it contains larger variance compared charades-ego. [Low priority]} 
%\TNnote{For space, can make this table smaller (that's why I changed headers to $M^{xyz}$ and attach the 2nd ablation table to the left/right.} 
%\YLnote{try to make Table 2 and 3 stand in one row side by side, but it looks very compact.}
%\KGnote{i think it would be good as single column. shorten dataset names?}
%\YLnote{May update epic-55 results with a new train/val split from LFB and AVslowfast}. Keep the old split as the results are similar.} 
%\TNnote{See notes in baselines section. Split this table into just the baselines, and then a separate table with the crosses and ticks for the ablation experiments. No need to mix them up here.} \YLnote{Yeah, we can split it later}}
\label{tb:different_aux}
\end{table}



Table~\ref{tb:different_baseline} shows the validation performance of different pre-training strategies. %As shown
\emph{Third-only} benefits from strong initialization from large-scale video pre-training and greatly outperforms models trained from \emph{Scratch}.
\emph{First-only} performs very poorly despite being %Though
pre-trained on the largest available egocentric dataset, %(Epic-Kitchens-100~\cite{epic-100}), % First-only still has much worse performance 
%\TN{but performs} much worse on Charades-Ego compared to Third-only,% which pre-trained on Kinetics, which suggests that the third-person pre-training is still palying the key role in egocentric domain. 
indicating that increasing scale alone is not sufficient---the diversity of scenes and activities in %does not pre-training ego-models is not limited exclusively by the scale of egocentric datasets---
third-person data plays a significant role in feature learning as well. 
% \TNnote{Little bit contradictory to when we said on Charades, training on Charades first person was better than training on Charades Third person.} \KGnote{it also contradicts itself? because it does show that perf is limited by scale of even largest existing egocentric datasets?}
\emph{Domain-adapt} and \emph{Joint-embed} both learn viewpoint invariant features using additional unlabeled egocentric data. % introduce loss terms that conflict with the action recognition objective as the instances in the two domains do not share any action labels 
However, the large domain gap and small scale of the paired dataset limit improvements over \emph{Third-only}. % \emph{Domain-Adapt} could not adapt well from Kinetics to the ego domain due to the large domain gap, while \emph{Joint-embed} is limited in the scale and scenario of the paired dataset.
%As a result, these methods perform slightly worse than \emph{Third-only} on most metrics.
%\YL{only perform similarly with \emph{Third-only}}.
%Lastly, 
Our Ego-Exo method achieves the best %\KG{overall}
results on both Charades-Ego and EPIC-Kitchens. The consistent improvements (+1.54\% mAP on Charades-Ego, and +1.64\%/+1.97\% on EPIC verbs/nouns) over Third-only demonstrate the effectiveness of our proposed auxiliary egocentric tasks during pre-training.  This is a key result showing the impact of our idea. %\TNnote{Check numbers now that it's 3-run avg.} 
%\KGnote{do we need to acknowledge third-only is best on top-5 nouns?} \TNnote{and top-5 verbs. YL, Is this an artifact of the smaller validation set on EPIC?} \YLnote{I think it's caused by variance. Plan to updated by 3-run averaging. Let's see how it goes.}
%\YLnote{Updated with 3-run average.}

% \KGnote{when giving our results, let's be sure to highlight where we can conclude that even with the most available egocentric video, our method is helping (if we can).  To counter the argument ``but there are large ego video datasets now".  Maybe this is most apparent in Charades-Ego, where pre-training for EPIC, say, wouldn't do much help?}
% \YLnote{(1) We could show improvements on Epic-100. (2) compare Ego-exo with a Epic-100 pre-trained model on the results on Charades-Ego?} \TNnote{Even EPIC-55 would be more than enough to prove our point, plus it won't raise questions about why we don't use EPIC-100 for everything.}

Fig~\ref{fig:classwise} shows a class-wise breakdown of performance on Charades-Ego compared to the \emph{Third-only} baseline. Our pre-training strategy results in larger improvements on classes that involve active object manipulations. % \KGnote{which baseline is this against?} 
% \TNnote{Here is a good place for some qualitative results + discussion (instead of saving it for an independent section later on).}\KGnote{agreed.}

\begin{figure*}[t!]
\centering
\includegraphics[width=2.0\columnwidth]{figs/classwise-breakdown}
\vspace{-2mm}
\caption{\textbf{Class-level performance on Charades-Ego.} Our method significantly improves on several classes that focus on active object manipulations (green lines), and performs only marginally worse across most under-performing classes (red lines). 35 most/least improved classes (out of all 157 classes) are shown.
%\TNnote{If nothing meaningful to say, move to Supp.}
}
\vspace{-3mm}
\label{fig:classwise}
\end{figure*}


\subsection{Ablation studies}
% \YLnote{I combine this two small ablation sections into one}

\begin{table}[t]
\small
% \renewcommand\arraystretch{1.1}
% 	\begin{center}
\centering
\resizebox{\columnwidth}{!}{
	\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{l|c|cc|cc}
		%\hline
		    &  C-Ego & \multicolumn{2}{c|}{EPIC verbs} & \multicolumn{2}{c}{EPIC nouns} \\
		\cline{2-6}
		Methods	&  mAP  & top-1 & top-5 & top-1 & top-5	\\
		\hline
        Third-only  &  24.69 & 61.19 & 87.49 & 46.18 & 69.72  \\
        Third-only +aux &  25.00 & 62.36 & 87.72 & 46.59 & 68.33 \\
        {$\Delta$} & \textit{+0.31} & \textit{+1.17} & \textit{+0.23} & \textbf{\textit{+0.42}} & \textit{-1.39} \\
        \hline
        Ego-Exo  & 26.23 & 62.83 & 87.63 & 48.15 & 70.28 \\
        Ego-Exo +aux & 27.47 & 64.26 & 88.45 & 48.39 & 70.68\\
        % {$\Delta$} & \textbf{\textit{+1.16}}  &	\textbf{\textit{+1.17}} &	\textbf{\textit{+1.38}} &	\textbf{\textit{+1.41}} &	\textbf{\textit{+1.17}} \\
        {$\Delta$} &  \textbf{\textit{+1.24}} &  \textbf{\textit{+1.43}} &  \textbf{\textit{+0.82}} & \textit{+0.24} & \textbf{\textit{+0.40}} \\
		\hline				
	\end{tabular}
% 	\end{center}
}
\vspace{-2mm}
\caption{\textbf{Effect of Ego-Exo losses during fine-tuning.} Adding distillation losses during fine-tuning improves performance for both models, and results in a larger performance gain for our Ego-Exo pre-trained models. \cc{Values are averaged over 3 runs.}
%\TNnote{Awkward but I changed to + aux since I want to formally define Ego-Exo* and Ego-Exo+ later.} \YLnote{Looks good}
}
\vspace{-3mm}
%Results of methods with(*) and without adding auxiliary task during fine-tuning on Charades-Ego and Epic-Kitchen datasets with Slow-only model. 
\label{tb:add_loss_to_ego}
\end{table}


%\subsection{\TN{Impact of auxiliary ego tasks}}
\paragraph{Impact of auxiliary ego-tasks.}
%\noindent\textbf{Impact of auxiliary ego-tasks.}
We next analyze the impact of each auxiliary egocentric task in our Ego-Exo framework. % the Third-only baseline. %method as the compared baseline which is pre-trained on Kinetics-400 without any auxiliary egocentric tasks. 
As shown in Table~\ref{tb:different_aux}, adding the \emph{Ego-Score} task improves performance %over the baseline 
on both EPIC-Kitchens tasks, while adding \emph{Object-Score} and \emph{Interaction-Map} consistently improves all results. %on both Charades-Ego and Epic-Kitchen datasets.
This reveals that despite varying structure and semantics, these scores capture important underlying egocentric information to complement %and successfully supplement useful egocentric cues for the 
third-person pre-training, and further boost performance when used together. %Finally, incorporating three auxiliary tasks together further boost the overall performance.


Fig~\ref{fig:retrieval-swatch} shows instances from Kinetics based on our auxiliary pseudo-label scores combined with the weights in Eqn~\ref{eqn:loss}. %sorted by the combination of these task scores, following the same weighting as Eqn~\ref{eqn:loss}. 
% \YLnote{I feel talking about "combination of these task scores using weighting in Eqn~\ref{eqn:loss}" may cause confusion if we have combination of scores for training.} % Agreed
Our score is highest for object-interaction heavy activities (e.g., top row: knitting, changing a tire), while it is low for videos of broader scene-level activities (e.g., bottom row: sporting events). Note that these videos are not in the egocentric viewpoint---they are largely third-person videos from static cameras, but are \emph{ego-like} in that they prominently highlight important features of egocentric activity (e.g. hands, object interactions).



% \TNnote{Good place for another qualitative result --- the venn diagram if it makes sense.}
% TN: Added retrieval results instead of venn diagram. That could go in Supp?

% \subsection{\TN{Adding distillation loss during fine-tuning}}
\vspace{-2mm}
\paragraph{Adding auxiliary ego-tasks during fine-tuning.} 
%\noindent\textbf{Adding auxiliary ego-tasks during fine-tuning.}
% Our auxiliary egocentric loss could also be extended to the downstream egocentric datasets. Similar scheme of using distillation on fine-tuning has been explored in semi-supervised learning~\cite{chen2020big}.
Our auxiliary losses may also be added \emph{after} pre-training, for fine-tuning downstream egocentric models similar to prior semi-supervised learning work~\cite{chen2020big}. %\YLnote{To BO, I add the reference here}
% \cc{This setting is less desirable as it would require extra model components during fine-tuning, and the auxiliary losses may interfere with the objective if not carefully tuned, but can benefit tasks like activity recognition.} 
% \YLnote{I am thinking if we want to explicitly show dislike as it has also been considered as one setting of our Ego-Exo}. 
% \KGnote{``This setting is less desirable..." do we need to get into that?  maybe keep it simple.}
% TN: Ok, makes sense.
% For the auxiliary tasks on egocentric datasets, Ego-Score is likely to be 1 for all egocentric videos and Object-Score may already be covered by the interaction action labels from egocentric datasets. Thus, Interaction-Map provides most supplementary knowledge for egocentric video understanding. Similar to the Interaction-map prediction for third-person dataset, we generate the corresponding interaction-map on egocentric datasets and then add the auxiliary loss $\mathbb{L}_{int}$ in Eqn~\ref{eq:int-map} during fine-tuning. 
We re-introduce our Interaction-Map loss $\mathbb{L}_{int}$ (Eqn~\ref{eq:int-map}) %while fine-tuning our models 
for downstream egocentric training. We do not include Ego-Score (which is trivially high for all videos) and Object-Score (which is subsumed in the interaction label for this setting) %for simplicity and 
as their impact %on downstream performance
after pre-training was minimal. 

% \TNnote{@YL: Check if impact is actually minimal}. \YLnote{Yes, I have validated object-score on charades-ego/epic is not helping. Ego-score has a average scores of 0.97 on epic.}
% \KGnote{that one is shaky explanation} \TNnote{Agreed about shaky explanation for both (more for object score). Did we try them and they did worse? YL, any other explanation? The object score is a soft-score that has extra imagenet info beyond the charades label for sure.} \YLnote{Yes, I tried object-score on Charades-Ego, no improvements found. I can conduct on Epic again, then we safely claim no improvements for object-score. For Ego-Score, we need to conduct on epic if we want. But I expect ego-score could be all near 1}.  \KGnote{to streamline this, is it the case that using all of them is no worse than using just InteractionMap?}
% Note that for egocentric video, the Ego-Score is likely trivial (videos are all egocentric), and the Object-Score is likely subsumed in the interaction label, \KGnote{that one is shaky explanation} thus we only consider the Interaction-Map loss.  
% \KGnote{if possible shorten up and merge the first two paras in this section.}




Table~\ref{tb:add_loss_to_ego} shows that while both the baseline and our method further improve by adding the auxiliary task during fine-tuning, 
our improvements (Ego-Exo + aux) are larger, especially on Charades-Ego. %\KGnote{is Ego-Exo + aux the same as Ego-Exo* below?} \YLnote{yes, so now we a formal definition in the beginning of Sec 4.3. but I am neutral to still use Ego-Exo* or Ego-Exo+aux.} 
This is likely because 
% Moreover, the improvements to Ego-Exo %from Ego-Exo* over Ego-Exo 
% are larger than improvements to Third-only, especially on Charades-Ego. This is likely because %pre-training of the interaction-map prediction heads in the auxiliary task on large-scale third-person dataset provide 
our distillation heads benefit from training to detect hands and objects in large-scale third-person video prior to fine-tuning for the same task on downstream ego-datasets.
% While adding auxiliary task for Third-only only improves marginally due to the limit number of samples in Charades-Ego. This validates the necessity and effectiveness of adding auxiliary egocentric tasks for third-person pre-training in Ego-Exo framework. % TN: No need for a 2nd conclusion

\begin{table}[tb]
\small
\renewcommand\arraystretch{1.1}
	\begin{center}
%	\setlength{\tabcolsep}{3.5pt}
	\begin{tabular}{l|c}
% 		\hline
		Method	& mAP	\\
		\hline
		ActorObserverNet~\cite{sigurdsson2018actor} & 20.0 \\
		SSDA~\cite{choi2020unsupervised} & 23.1 \\
        I3D~\cite{choi2020unsupervised} & 25.8 \\
	    \hline
        SlowFast~\cite{slowfast} & 25.93 \\
        Ego-Exo & 28.04 \\
        Ego-Exo* & 29.19 \\
        Ego-Exo*-R101 & \textbf{30.13} \\
        \hline
	\end{tabular}
	\end{center}
\vspace{-5mm}
\caption{\textbf{Comparison to prior work on Charades-Ego.} Despite having no access to paired egocentric data, our model outperforms specialized joint-embedding and domain adaptation based methods.  %, without access to paired egocentric data. 
%\TNnote{Can we have an Ego-Exo*-R101 here for completeness?}}  %SlowFast~\cite{slowfast}, Ego-Exo, and Ego-Exo* use SlowFast-ResNet50 as the backbone model. \KGnote{unclear, should we be emphasizing that the others use something different/stronger?}}
% TN: Already mentioned in Sec. 4.3
}
\vspace{-3mm}
\label{tb:charades-ego-results}
\end{table}

\subsection{Comparison with state-of-the-art}
% \YLnote{It's also possible to have a Ego-Exo with ResNet-101 if we want to beat all SOTA}
% \TNnote{If we can afford the cycles, I think anything is fair game for this subsection, especially if we're comparing against methods that have access to Audio etc.} \KGnote{yes definitely would win over certain reviewers.  and it's partly inconclusive to say ``we do pretty good but not as good as those that elected to use better backbone or more modalities."}
% \TNnote{We use SlowFast here. Say explicitly and in caption}
% \subsection{Results}
% \subsubsection{Action Recognition Results}
%-EGTEA



\begin{table*}[tb]
\small
%\renewcommand\arraystretch{1.1}
	\begin{center}
	\setlength{\tabcolsep}{4.5pt}
	\begin{tabular}{c|l|cccccc|ccc|ccc}
	%	\hline
	   & & \multicolumn{6}{c|}{Overall} & \multicolumn{3}{c|}{Unseen Participants} & \multicolumn{3}{c}{Tail Classes} \\
	   \cline{3-14}
	  &  & \multicolumn{3}{c|}{top-1} & \multicolumn{3}{c|}{top-5} &	\multicolumn{3}{c|}{top-1} & \multicolumn{3}{c}{top-1} \\
	   \cline{3-14}
	&	Methods &  verb & noun & \multicolumn{1}{c|}{actions} & verb & noun & actions & verb & noun & actions & verb & noun & actions \\
	% 	\cline{2-13}
	
		\hline
% 	\color{darkgray}{\textit{w/ audio}} &	\color{darkgray}{\textit{Epic-Fusion~\cite{epic-fusion}}} & \color{darkgray}{\textit{62.40}} & \color{darkgray}{\textit{46.50}} & \color{darkgray}{\textit{35.11}} & \color{darkgray}{\textit{88.74}} & \color{darkgray}{\textit{72.24}} & \color{darkgray}{\textit{55.17}} & \color{darkgray}{\textit{56.57}} & \color{darkgray}{\textit{41.78}} & \color{darkgray}{\textit{29.46}} & \color{darkgray}{\textit{29.41}} & \color{darkgray}{\textit{18.55}} & \color{darkgray}{\textit{13.47}} \\
	\color{darkgray}{{w/ audio}} &	\color{darkgray}{{Epic-Fusion~\cite{epic-fusion}}} & \color{darkgray}{{62.40}} & \color{darkgray}{{46.50}} & \color{darkgray}{{35.11}} & \color{darkgray}{{88.74}} & \color{darkgray}{{72.24}} & \color{darkgray}{{55.17}} & \color{darkgray}{{56.57}} & \color{darkgray}{{41.78}} & \color{darkgray}{{29.46}} & \color{darkgray}{{29.41}} & \color{darkgray}{{18.55}} & \color{darkgray}{{13.47}} \\
		\Xhline{2\arrayrulewidth}
	\multirow{7}{*}{w/o audio} &	TSN fusion~\cite{epic} &  58.43 & 46.54 & 32.79 & 87.27 & 72.49 & 53.12 & 52.04 & 42.09 & 26.30 & 24.76 & 14.91 & 10.41 \\
    	& TRN~\cite{zhou2018temporal} & 62.56 & 45.70 & 34.41 & 88.24 & 71.37 & 54.65 & 57.49 & 40.85 & 28.69 & 27.24 & 13.42 & 11.20 \\
		& TSM~\cite{lin2019tsm} & 65.51 & 48.48 & 37.58 & \textbf{89.39} & 73.46 & 58.04 & 59.66 & 43.16 & 30.41 & 29.76 & 15.84 & 13.15 \\
        \cline{2-14}
        & SlowFast~\cite{slowfast} & 63.89 & 49.66 & 37.42 & 88.71 & 74.99 & 58.17 & 57.37 & 44.31 & 29.71 & 33.57 & 22.57 & 16.55 \\
        & Ego-Exo & 64.08 & 50.59 & 38.38 & 88.57 & 74.82 & 59.04 & 57.42 & 46.18 & 31.41 & 32.87 & \textbf{22.98} & 16.30 \\
        & Ego-Exo* & 65.02 & \textbf{51.74} & 39.52 & 89.26 & 75.95 & 60.07 & 58.86 & \textbf{47.01} & 32.36 & 33.68 & 22.35 & 16.30 \\
        & Ego-Exo*-R101 & \textbf{66.07} & 51.51 & \textbf{39.98} & \textbf{89.39} & \textbf{76.31} & \textbf{60.68} & \textbf{59.83} & 45.50 & \textbf{32.63} & \textbf{33.92} & 22.91 & \textbf{16.96} \\
        \hline
	\end{tabular}
	\end{center}
\vspace{-5mm}
\caption{\textbf{Comparison on EPIC-Kitchens-100 action recognition test set.} Our method %outperforms the other methods
is best in all categories.
%SlowFast~\cite{slowfast}, Ego-Exo and Ego-Exo* use a SlowFast-R50 as the backbone model while Ego-Exo*-R101 use a SlowFast-R101. Note other methods use different backbones or more modalities. 
% \YLnote{make epic-fusion italics or gray}
%\KGnote{same comment as above, we can do them in a parallel way.}
%\KGnote{need some boldfaces, shading etc. like in other table.}
}
\vspace{-4.5mm}
\label{tb:epic-100-results}
\end{table*}



%In this section,
Finally, we compare our method with state-of-the-art models, %from prior work
many of which use additional modalities (flow, audio) compared to our RGB-only models. %on several datasets, including Charades-Ego~\cite{charades-ego}, Epic-Kitchen~\cite{epic} and Epic-Kitchen-100~\cite{epic-100}. Note that 
We include three competitive variants of our model using SlowFast~\cite{slowfast} backbones: (1) \textbf{Ego-Exo} uses a ResNet50 backbone; (2) \textbf{Ego-Exo*} additionally incorporates our auxiliary distillation loss during fine-tuning.\footnote{Same as Ego-Exo + aux in Table~\ref{tb:add_loss_to_ego}, but here with a SlowFast backbone} (3) \textbf{Ego-Exo*-R101} %uses a ResNet101 backbone and also our fine-tuning losses. 
further uses a ResNet-101 backbone.
% \YLnote{I would prefer Ego-Exo*-R101 a little more as it is clearer when looking at the Table and introduces less additional magic symbols.} % Makes sense!
%and  an RGB-only SlowFast model~\cite{slowfast} as our video backbone when training the baseline and our method. 
% Importantly, the existing methods may use %a stronger backbone or 
% additional modalities (flow, audio). % \YLnote{remove stronger backbone as we now also conduct R101}




\vspace{-1mm}
\paragraph{Charades-Ego.}
%\vspace{1mm}
%\noindent\textbf{Charades-Ego.}
Table~\ref{tb:charades-ego-results} compares our Ego-Exo method with %the current 
existing methods. Our Ego-Exo and Ego-Exo* yield state of the art accuracy, improving performance over the strongest baseline by +2.11\% and +3.26\% mAP. We  observe large performance gains over prior work, %previous methods, 
including ActorObserverNet~\cite{sigurdsson2018actor} and SSDA~\cite{choi2020unsupervised}, which use joint-embedding or domain adaptation approaches to transfer third-person video features to the first-person domain. In addition, unlike the competing methods, our method does not require any egocentric data which is paired or shared category labels with third-person data during pre-training.
%\KGnote{Do we want to call attention to which use paired labels / shared category labels at this point?  or let it be a column in table with checkbox? risk is that we have access to off-the-shelf models trained in other ways.} 
%\YLnote{Also another risk is that they may use less labels than us on ego videos. So I slightly prefer not to add a column as the setting is always not fair but we are better than them. }





\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/retrieve-4-blur}
\vspace{-4mm}
\caption{\textbf{Kinetics instances sorted by Ego-Exo scores.} Our task scores are maximum for videos that prominently feature hands/objects in view (top row), and minimum for scenes devoid of human-centered activity (bottom row). 
% \TNnote{Can slip in CAM heatmaps in this fig itself.} \YLnote{let's have CAM in Supp}
% \YLnote{Will it cause some confusions as we don't have Ego-Exo score in the method and we are not assigning weights to instances during training? Do we need to clarity it ?} % Showing all 3 scores now
}
 \vspace{-3mm}
\label{fig:retrieval-swatch}
\end{figure}


\vspace{-3mm}
\paragraph{EPIC-Kitchens.} 
%\vspace{1mm}
%\noindent\textbf{EPIC-Kitchens.}
Table~\ref{tb:epic-55-results} compares our method to state-of-the-art models on the EPIC-Kitchens test set. %First, 
Ego-Exo and Ego-Exo* %methods
%\KGnote{is the star one defined now?} \YLnote{Ego-Exo* is first defined in the ablation study} 
consistently improve over SlowFast (which shares the same backbone architecture) %the apples-to-apples baseline SlowFast % apples to apples baseline sounds funny
for all %label %verb / noun / action 
categories on both seen and unseen test sets.
Epic-Fusion~\cite{epic-fusion} uses additional optical flow and audio modalities together with RGB, yet % on Epic videos during fine-tuning,
Ego-Exo outperforms it on the top-1 metric for all categories. %on both seen and unseen test sets.  
AVSlowFast~\cite{xiao2020audiovisual} also utilizes audio, but is outperformed by our model with the same backbone (Ego-Exo*-R101) %and a stronger backbone (SlowFast-R101), yet Ego-Exo* outperforms it 
on the S1 test set.\footnote{Table~\ref{tb:epic-55-results} compares existing methods under a controlled setting: using a single model with RGB or RGB+audio as input, and only Kinetics/ImageNet for pre-training.  Other reported results on the competition page may use extra modalities, larger pre-training datasets, or model ensemble schemes (e.g. the top ranking method ensembles 8 models).}
On %the extended dataset 
\textbf{EPIC-Kitchen-100}~\cite{epic-100}, as shown in Table~\ref{tb:epic-100-results}, Ego-Exo consistently improves over the SlowFast baseline on all evaluation metrics, and Ego-Exo*-R101 outperforms \emph{all} existing %compared
state-of-the-art methods.
%\TNnote{Merge with previous EPIC?}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\setlength{\tabcolsep}{3pt}
	\begin{tabular}{c|l|cc|cc|cc}
	%	\hline
		&	& \multicolumn{2}{c|}{verbs} & \multicolumn{2}{c|}{nouns} & \multicolumn{2}{c}{actions}\\
		\cline{2-8}
	\textbf{S1 (seen)}	& Methods	&   top-1 & top-5 & top-1 & top-5 & top-1 & top-5	\\
		%\hline
		%&  & & & & & &  \\
		\hline
% 		\textit{Epic-Fusion}~\cite{epic-fusion} & \textit{64.75} & \textit{\textbf{90.70}} & \textit{46.03} & \textit{71.34}  & \textit{34.80} & \textit{56.65} \\
% 		\textit{AVSF-R101}~\cite{xiao2020audiovisual} & \textbf{\textit{65.70}} & \textit{89.50}  & \textbf{\textit{46.40}}  & \textit{\textbf{71.70}}  & \textbf{\textit{35.90}}  & \textit{\textbf{57.80}}  \\
% 	 \color{darkgray}{\textit{\multirow{2}{*}{w/ audio}}}	& \color{darkgray}{\textit{Epic-Fusion}~\cite{epic-fusion}} & \color{darkgray}{\textit{64.75}} & \color{darkgray}{\textit{\textbf{90.70}}} & \color{darkgray}{\textit{46.03}} & \color{darkgray}{\textit{71.34}}  & \color{darkgray}{\textit{34.80}} & \color{darkgray}{\textit{56.65}}\\
% 	&	\color{darkgray}{\textit{AVSF-R101}~\cite{xiao2020audiovisual}} & \color{darkgray}{\textbf{\textit{65.70}}} & \color{darkgray}{\textit{89.50}}  & \color{darkgray}{\textbf{\textit{46.40}}}  & \color{darkgray}{\textit{\textbf{71.70}}}  & \color{darkgray}{\textbf{\textit{35.90}}}  & \color{darkgray}{\textit{\textbf{57.80}}} \\
	 \color{darkgray}{{\multirow{2}{*}{w/ audio}}}	& \color{darkgray}{{Epic-Fusion}~\cite{epic-fusion}} & \color{darkgray}{{64.75}} & \color{darkgray}{{\textbf{90.70}}} & \color{darkgray}{{46.03}} & \color{darkgray}{{71.34}}  & \color{darkgray}{{34.80}} & \color{darkgray}{{56.65}} \\
	&	\color{darkgray}{{AVSF-R101}~\cite{xiao2020audiovisual}} & \color{darkgray}{\textbf{{65.70}}} & \color{darkgray}{{89.50}}  & \color{darkgray}{\textbf{{46.40}}}  & \color{darkgray}{{\textbf{71.70}}}  & \color{darkgray}{\textbf{{35.90}}}  & \color{darkgray}{{\textbf{57.80}}} \\
		\Xhline{2\arrayrulewidth}
		%\midrule
	\multirow{6}{*}{w/o audio} &	TSN fusion~\cite{epic} & 48.23 & 84.09 & 36.71 & 62.32 & 20.54 & 39.79  \\
	&	RU-LSTM~\cite{furnari2019would} & 56.93 & 85.68 & 43.05 & 67.12 & 33.06 & 55.32 \\
		\cline{2-8}
    &    SlowFast~\cite{slowfast} & 64.57 &	89.67&	45.89&	69.50&	34.67&	54.47 \\
    &    Ego-Exo &  65.84&	89.91&	46.68&	70.30&	36.00&	54.90\\
    %&    Ego-Exo* & \textbf{66.19} &	89.97&	47.16 &	70.42&	36.45 &	55.44  \\
     &    Ego-Exo* & \textbf{66.19} & 90.11 & 47.21 & 70.08 & 37.04 & 55.91  \\
    &    Ego-Exo*-R101 & 65.97 & \textbf{90.32} & \textbf{47.99} & \textbf{70.72} & \textbf{37.09} & \textbf{56.32} \\
        \hline
        \hline
    \textbf{S2 (unseen)} & & & & & & &  \\
    \hline
%     \color{darkgray}{\textit{\multirow{2}{*}{w/ audio}}} &    \color{darkgray}{\textit{Epic-Fusion}~\cite{epic-fusion}} & \color{darkgray}{\textit{52.69}} & \color{darkgray}{\textit{79.93}} & \color{darkgray}{\textit{27.86}} & \color{darkgray}{\textit{53.87}} & \color{darkgray}{\textit{19.06}} & \color{darkgray}{\textit{36.54}} \\
% 	&	\color{darkgray}{\textit{AVSF-R101}~\cite{xiao2020audiovisual}} & \color{darkgray}{\textit{\textbf{55.80}}} & \color{darkgray}{\textit{\textbf{81.70}}} & \color{darkgray}{\textit{\textbf{32.70}}} & \color{darkgray}{\textit{\textbf{58.90}}} & \color{darkgray}{\textit{\textbf{24.00}}} & \color{darkgray}{\textit{\textbf{43.20}}} \\
	 \color{darkgray}{{\multirow{2}{*}{w/ audio}}} &    \color{darkgray}{{Epic-Fusion}~\cite{epic-fusion}} & \color{darkgray}{{52.69}} & \color{darkgray}{{79.93}} & \color{darkgray}{{27.86}} & \color{darkgray}{{53.87}} & \color{darkgray}{{19.06}} & \color{darkgray}{{36.54}} \\
	&	\color{darkgray}{{AVSF-R101}~\cite{xiao2020audiovisual}} & \color{darkgray}{{\textbf{55.80}}} & \color{darkgray}{{\textbf{81.70}}} & \color{darkgray}{{\textbf{32.70}}} & \color{darkgray}{{\textbf{58.90}}} & \color{darkgray}{{\textbf{24.00}}} & \color{darkgray}{{\textbf{43.20}}} \\
		\Xhline{2\arrayrulewidth}
	\multirow{6}{*}{w/o audio} &	TSN fusion~\cite{epic} &  39.40 & 74.29 & 22.70 & 45.72 & 10.89 & 25.26 \\
	&	RU-LSTM~\cite{furnari2019would} & 43.67 & 73.30 & 26.77 & 48.28 & 19.49 & 37.15 \\
        \cline{2-8}
    &    SlowFast~\cite{slowfast} & 53.91 &	80.81 &	30.15 &	55.48 &	21.58 &	37.56 \\
    &    Ego-Exo &  54.11 & 	80.37 &	30.83 & 57.08 &	21.20 & 38.34\\
   % &    Ego-Exo* & 53.53 &	79.65 &	30.32 &	57.15 &	21.71 &	38.14  \\
    &    Ego-Exo* & 53.88 & 80.51 & 31.44 & 57.60 & 22.02 & 39.13 \\
    &    Ego-Exo*-R101 & \textbf{55.34} & \textbf{81.46} & \textbf{31.72} & \textbf{58.25} & \textbf{22.81} & \textbf{40.18} \\
        \hline
	\end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Comparison to prior work on EPIC-Kitchens (test set).} 
%S1 evaluates unseen videos in seen kitchens; S2 evaluates unseen videos in unseen kitchens. \YLnote{remove to save space}
Methods in \textcolor{darkgray}{gray} use additional audio modality information. Our method outperforms all methods that use consistent modalities in both settings, and is competitive with models that benefit from audio stream inputs. 
%\TNnote{don't need italics now that you've separated them well.}
%\TNnote{I would order these TSN, RULSTM | EPIC-Fusion, AVSF | SF Ours ours ours, and then put both audio rows in grey color (still include the bolds, but keep them grey so its clear. Same for the other table. Use a darker grey though :P}
%\YLnote{No preference on the italics or grey. But I would prefer keep the current order, as it's clearer to divide into two sets and the boldface for ego-exo is for the set w/o audio}\KGnote{I like the idea of gray backgrounds on the audio rows, ideally even with a vertical label that says ``+audio" on the left hand side.  and since we have another horiz line between RULSTM and SlowFast, we should make it explicit that we are bolding for best visual+audio and best visual-only methods?  and point out all these formatting things, like the orange too. or consider dropping the orange to be less complicated.}
%\YLnote{Oh, orange just indicates my changes, so I will remove that color :)}
% TN: We don't need to describe backbones now that we were pretty up front about it in the beginning of the section
% SlowFast~\cite{slowfast}, Ego-Exo and Ego-Exo* use SlowFast-R50 as the backbone model, while AVSF-R101~\cite{xiao2020audiovisual} and Ego-Exo*-R101 use SlowFast-R101. Note that Epic-Fusion~\cite{epic-fusion} and AVSF-R101~\cite{xiao2020audiovisual} use additional audio stream.
%\KGnote{I see the audio ones are in italics - make their numbers in italics too?  and put a boldface for w/audio winner and w/o audio winner?  could put the horiz line under the audio ones to separate from non-audio ones?  we need this table to show a boldface set for our method clearly.} \YLnote{Q: what's best name to add the ResNet101 row? Any suggestions. Still working on pushing the Ego-Exo*+R101 on s2.} \TNnote{Ego-Exo+?}
}
\vspace{-4mm}
\label{tb:epic-55-results}
\end{table}



% \paragraph{Action anticipation task}

% \subsection{Ablation Studies}

% In this section, we conduct different ablation studies on Charades-Ego and validation set of Epic-Kitchens~\cite{epic}. We use Slow-only model~\cite{slowfast} with ResNet-50 as backbone for ablation experiments. --- TN: mention this explicitly in each table caption.


% \KGnote{somewhere -- a vanilla domain adaptation method as a baseline?}
% \YLnote{could add in Table~\ref{tb:different_pre-train} and Sec 4.3}

% \YLnote{Move to appendix}
% \paragraph{Effects of interaction-map position; hand-map and object-map ablation} 

% Table~\ref{tb:different_stage}: Ablation studies of applying interaction-map prediction on different stages of backbone (Stage3, Stage4, Stage4 of ResNet).

% \begin{table}[t]
% \small
% \renewcommand\arraystretch{1.1}
% 	\begin{center}
% 	\setlength{\tabcolsep}{3.5pt}
% 	\begin{tabular}{c|c|c}
% 		\hline
% 		Stage	& Charades-Ego mAP  & Epic-kitchen	\\
% 		\hline
%         S3 &  \\
%         S4 & \\
%         S5 & \\
%         S4 + S5 & \\
% 		\hline				
% 	\end{tabular}
% 	\end{center}
% \caption{Applying interaction-map prediction on different stages of backbone.}\YLnote{Appendix}
% \label{tb:different_stage}
% \end{table}

% \paragraph{Results of comparing pre-trained models under fix-backbone setting.} [optional?]

% \TNnote{Low priority:}
% % \subsection{Other egocentric tasks}

% Results on other downstream ego tasks

% \textbf{Action Anticipation}

% -Epic-Kitchen-55

% -Epic-Kitchen-100

% \textbf{Unsupervised Domain Adaptation Action Recognition}

% -Epic-Kitchen-100

% \subsection{Qualitative Analysis} \TNnote{Merge qual results with previous results sections. See notes in exp sections.}

% \paragraph{Kinetics examples with auxiliary ego labels.}
% Examples with highest and lowest ego-scores.

% Examples with object-scores

% Examples with and without hand-object interactions

% \paragraph{TSNE visualization of pre-trained features.} k400-pre-train, DA pre-train and Ego-Exo pre-train.

% \paragraph{CAM visualization of the final models.} Compare baseline, DA pre-train and Ego-Exo.

% \paragraph{Per-class performance comparison.} Compare verb and noun per-class accuracy among baseline and Ego-Exo. 

% \TNnote{See google doc for some qual items. TODO: retrieval for each metric. TODO: CAM}

% \KGnote{let's include some qualitative results and per-class analysis etc., to break up all the tables.  Anything clever with Tsne on the pre-trained Kinetics vs. pre-trained ours (vs domain adaptation) features?  Showing examples of the exo videos (frames) deemed most vs least egocentric / examples showing hands+objects?  classes that most benefit from our approach and those that are least changed in accuracy vs. baseline? venn diagram figs like the epic fusion paper where each dot is a class or modality?}
% \YLnote{About venn diagram, are we trying to compare (ego-exore, object-score and interaction-map) or (baselines and ego-exo)?}


==> Ego-Exo_CVPR21 (ArXiv)_4:14:2021/sections/intro.tex <==
\section{Introduction}

\begin{textblock*}{\textwidth}(0cm,-16cm)
\centering
In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR), 2021. 
\end{textblock*}


% Egocentric video understanding is very popular recently. Difference between Third-person and egocentric: a unique viewpoint, reflecting agent’s attentions and interactions. Many different methods are explored, especially deep learning methods~\cite{}.

Egocentric video captured by wearable cameras offers a unique perspective into human behavior.  It is the subject of a recent surge in research interest in first-person activity recognition~\cite{epic-fusion,zhou2015temporal}, anticipation~\cite{furnari2020rolling,abu2018will}, and video summarization~\cite{lee2015predicting,yonetani2016visual,del2016summarization}
%accompanied by the release of of ego-video datasets and benchmark challenges
%KG here I think we don't want to make the point first that big ego datasets are emerging; it's counter to the next piece of text.
%~\cite{pirsiavash2012detecting,charades-ego,epic,li2018eye,epic-100}, 
with many valuable future applications in augmented reality and robotics.
Compared to third-person videos, %egocentric video is strongly tied to the camera wearer's intentions and activities. The videos 
egocentric videos show the world through a distinct viewpoint, encode characteristic egocentric motion patterns due to body and head movements, and have a unique focus on hands, objects, and faces, driven by the camera wearer's attention and interaction with their surroundings. 


%\KGnote{This seems like an abrupt jump - we say ego is special, but we then say third person has the right signals.  how about first raise it as a problem: third-person video is better understood at this stage, yet has very different viewpoint and lacks the characteristics... BUT, nonetheless, people can understand how to translate...}
%\KGnote{do we have a conceptual angle besides ``there isn't enough labeled first-person video?" maybe we can recall the developmental learning story}%


However, these unique properties also present a fundamental challenge for video understanding.
On the one hand, learning models purely from egocentric data are limited by dataset scale. Current egocentric video datasets are small (e.g., 90k clips in EPIC-Kitchens-100~\cite{epic-100} vs.~650k in Kinetics-700~\cite{kinetics}) and lack diversity (e.g., videos only in kitchen scenes). %Moreover, they do not benefit from the egocentric signals embedded in third person video.
% \YL{The benchmarks in Charades-Ego~\cite{charades-ego} also demonstrates that only taking a third-person pre-trained model has a significant drop compared to using the first-person labeled data. (Fig~\ref{fig:comp_pre-train} Add a qualitative comparison of k400 pre-trained features and ego-exo pre-trained features.) } 
On the other hand, a purely exocentric approach that uses more readily available third-person %images or 
video---the status-quo for pre-training video models~\cite{slowfast,tsn,zhou2018temporal,nonlocal}---ignores the unique properties %features
of egocentric video and faces a major domain mismatch.
Prior work has shown that this latter strategy, though popular, is insufficient: pre-training egocentric action recognition models with third-person data alone produces significantly worse results than pre-training with first-person data~\cite{charades-ego}.
% \KGnote{how to convey concretely that this is insufficient, e.g., citing past results failing to benefit from 3rd person pre-training for 1st person results?} \TNnote{$\uparrow$ Good point. No one really complains about using Kinetics... We might be able to find an experiment on EGTEA+ that had better performance by pre-training on EPIC vs. Kinetics?}
In an attempt to bridge the domain gap, prior work explores traditional embedding learning~\cite{sigurdsson2018actor,yu2019see} or domain adaptation approaches~\cite{choi2020unsupervised}, but they require \emph{paired} egocentric and third-person videos that are either concurrently recorded or annotated for the same set of activities, which are difficult to collect and hence severely limit their scope.
% \KGnote{CHECK--do these all used paired data?} TN: I've referred to paired as sharing label space too. Only choi2020unsupervised doesn't use paired

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figs/concept_blur}
% \caption{qualitative comparison of k400 pre-trained features and ego-exo pre-trained features
%\vspace{-0.5mm}
\caption{\textbf{Main idea.} We extract key egocentric signals from large-scale third-person data and distill them into the video backbone during pre-training to guide feature learning for egocentric video tasks with wearable camera video.}
\vspace{-4.5mm}
\label{fig:main-idea}
\end{figure}


%Prior work has attempted to bridge this gap using traditional embedding learning approaches~\cite{sigurdsson2018actor,yu2019see,choi2020unsupervised} but require paired egocentric and third-person videos, severely limiting their scope.
% \TNnote{YL, check if this is right? What is actually wrong with domain adaptation methods that don't require paired data?}
% \YLnote{If we are talking about domain adaptation from exo to ego specifically, I don't find any other works besides~\cite{choi2020unsupervised}. For DA, I think it doesn't use the labels of ego datasets, so the results are worse than finetuning on ego datasets in practical.  }

%...not purely data availability, also conceptual...

%Despite these differences, 
Despite their differences, we hypothesize that the exocentric view of activity should in fact inform the egocentric view.   First, humans are able to watch videos of other people performing activities and map actions into their own (egocentric) perspective; babies in part learn new skills in just this manner~\cite{meltzoff1988imitation,premack1978does}.
% Found the perfect body of work to cite: http://ilabs.washington.edu/meltzoff/pdf/99Meltzoff_BornToLearn.pdf
Second, exocentric video is not devoid of person-centered cues.  For example, a close-up instructional video captured from the third-person view may nonetheless highlight substantial hand-object interactions; or video captured with a hand-held phone may follow an event (e.g., a parade) as it unfolds with attentional cues related to a head-mounted camera.  %%%\KGnote{not sure if these are strong enough examples, but trying to foreshadow our approach and flesh out more the motivation.}

 % Prior work has attempted to learn this mapping in the context of paired egocentric and third-person video~\cite{sigurdsson2018actor,yu2019see,choi2020unsupervised}
%  of how intelligent agents (people) first learn by watching other people do stuff and then figure out how to map that to themselves (ego)?  Trying to balance the purely practical motivation, which is still good, with some additional academic aspect.}

% Deep learning methods usually need a large amount data for training, however, current Popular egocentric video datasets~\cite{} are much smaller than third-person datasets~\cite{}. For example, Kinetics, Epic-Kitchen XX. 
% \begin{itemize}
%     \item So similar to ImageNet pre-training are an ubiquitous strategy for many different tasks~\cite{}, it's also very common to finetune from a pre-trained model on large-scale third-person dataset for ego datasets. However, the pre-trained model still focuses on the third-person domain. 
%     \item To explicitely transfer between third-person and first-person videos, Charades-Ego provides a dataset to jointly model first and third-person videos, but it's limited in the scale and paired setting. 
%     \item There is lack of a better way to better utilize large-scale third-person dataset for egocentric video understanding.
% \end{itemize} 
%Given the significance of both viewpoints, this raises the question: 

Building on this premise, in this work we ask: \emph{``How can we best utilize current video datasets to pre-train egocentric video models?''}  Our key idea is to discover latent signals in third-person video that approximate egocentric-specific properties.  To that end, we introduce a feature learning approach in which ego-video features are guided by both exo-video activity labels and (unlabeled) ego-video cues, to better align traditional third-person video pre-training with downstream egocentric video tasks.
%third-person video offers latent signals to help understand first person activity.
% In this paper, we propose \textit{\textbf{Ego-Exo}} to introduce novel approaches to better pre-training on large-scale third-person dataset and then transfer visual representation to ego datasets. The main idea is to have a better ego-specific exo-pre-trained model by  1) embedding ego-specific information during third-person pre-training 2). Encouraging pre-trained model focus on ego-related information and regions. 
%To address these issues, 

% Specifically, we first define several additional labels for video data and then transfer those knowledge by distillation during pre-training. 
% \begin{itemize}
%     \item what's the important information for ego videos? As we can see in the figure~\ref{}, egocentric videos are usually more driven by agent's motion, attention and interactions compared to third-person videos. Here we define two ego-specific labels for videos: \textit{ego-score} and \textit{object-score}. Ego-score is to measure the likelihood of a video as an egocentric video, which implicitly capture the underlying unique egocentric property. While object-score is to capture the dominating objects in the video, which explicitly focuses on the objects.
%     \item what's the important moments and regions for ego videos? As egocentric videos naturally have more hand-object interactions, the interaction moments and regions contains more important information for video understanding. Therefore, we define a temporal-spatial \textit{interaction-map} to represent the hand-object interactions in videos.
% \end{itemize}
% \TNnote{Let's not spell out all the different scores we're using right away. Details can go in approach}
% To transfer the knowledge encoded in the above ego-related labels, we introduce a general approach to embed the above information during third-person pre-training. Specifically, besides the original third-person action labels, we use loss distillation scheme to add additional tasks for knowledge transfer. 
% TN absorbed above
% We propose to upgrade the traditional third-person video pre-training framework by introducing \TN{these} key egocentric signals,
%into traditional third-person video model pre-training,
% to better align feature-learning with downstream egocentric video tasks. 
Specifically, we introduce a series of ego-inspired tasks that require the video model to be predictive of manipulated objects, spatiotemporal hand-object interaction regions, and general egocentricity.  Then we incorporate these tasks into training as knowledge-distillation losses to supplement  %the original 
an action classification pre-training objective on third-person video. See Fig.~\ref{fig:main-idea}.

% Note that not all third-person videos are required to contain hands or object interactions --- our distillation objective is meant to approximate the response of strong pre-trained egocentric models on third-person video data, meanwhile our model could still benefit from the diversity of actions and large scale in third-person datasets.
% Although the third-person videos do not always contain all our interested ego clues, most videos still contains hands or object interactions, as third-person video datasets are usually human-centric. So Our model also treats different third-person videos differently through by knowledge-distillation losses by using different soft targets.
% \TNnote{unclear how to justify using this for video without hands/objects if we're talking about labels, and not features.}
% \YLnote{Not sure if we want explicitly talking about video without hands/objects here? I think knowledge-distillation already handle those naturally through soft targets.}
% ^ TN: addressed in approach

% Advantages: 1) our method is still able to enjoy the as many as large-scale labeled third-person datasets, meanwhile embedded ego-specific information into the pre-trained model. 2) As our pre-trained model is focusing on the pre-training stage, it could be generally adopted by different egocentric datasets and tasks as initialization method without any modifications for the downstream models.
%As a result,
By design, our video models can continue to enjoy large amounts of labeled third-person training data, while simultaneously embedding egocentric signals into the learned features, making them a suitable drop-in replacement for traditional video encoders for egocentric video tasks.
% more suitable to finetune for downstream egocentric tasks. \YL{Moreover, once trained, our model can be used as an drop-in replacement for traditional video encoders %backbones
% in popular egocentric video models.}
%more complicated architectures that, for example, use multiple modalities.} %\YLnote{depending on if we will have AVSlowFast+Ego-Exo in the exps? Otherwise no need to emphasize multi-modality?}
% \KGnote{I'm not clear what's the difference of ``downstream ego tasks" and ``backbones" here.}  
Finally, our approach does not assume any paired or activity-labeled egocentric videos during pre-training; the egocentric signals are directly inferred from third-person video.
%\KG{assumes the egocentric pre-training videos are \emph{unlabeled} and \emph{unpaired} with the third-person data.}
% \KGnote{How can we make the point more clearly about how our idea differs from domain adaptation in concept?}
% TN: I added a reference to DA requiring paired/labeled data above.


% The experiments show that: 1). Our method leads to significant improvement on action recognition for different egocentric datasets. XX compared to training from scratch on Epic, XX compared to a Kinetics pre-trained  2) Our pre-trained model could also improves the performance for other egocentric tasks, like action anticipation and unsupervised action recognition in Epic.

Our experiments on three challenging egocentric video datasets show that our ``Ego-Exo'' framework learns strong egocentric feature representations %tailored to egocentric videos 
from third-person video. % collections. 
On Charades-Ego~\cite{charades-ego}, our model improves over models pre-trained on Kinetics---the standard % traditional
pre-training and fine-tuning paradigm---by +3.26 mAP, and outperforms methods that specifically aim to bridge the domain gap between viewpoints. % \TN{by Y\%.} 
Finally, our pre-trained model achieves state-of-the-art results on  EPIC-Kitchens-100~\cite{epic-100}, the largest available first-person dataset. % \YLnote{Let's see if we want to mention anticipation task based on the final results}
%, when used in conjunction with \TN{multi-modal models} \YLnote{(Let's see if AVSlowFast works well)}.

% \begin{itemize}
% \item Our proposed novel framework can learn feature representations tailored for egocentric videos from generic (third-person) video collections.

% \item Our models achieve improvements on action recognition, anticipation, etc. \KGnote{let's enumerate whatever it is, no etc.} compared to models pre-trained on Kinetics---the traditional pre-training and fine-tuning paradigm---and surpasses methods that specifically aim to bridge the domain gap between viewpoints. 

% \item Our pre-trained network serves as a drop-in replacement in more complicated egocentric video models and achieves state-of-the-art results when used in conjunction with them.
% \end{itemize}
% \YLnote{we could group into fewer items later after the exps are more ready}


==> Ego-Exo_CVPR21 (ArXiv)_4:14:2021/sections/method.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=1.95\columnwidth]{figs/arch_blur}
\vspace{-1.5mm}
\caption{\textbf{Ego-Exo framework}. To enhance traditional pre-training (left panel), we generate soft-labels for \emph{third-person videos} from a set of pre-trained egocentric models (top-right) that capture a variety of key egocentric signals (Sec~\ref{sec:tasks}), and we train distillation modules to approximate the responses of these models (bottom-right). 
% \TN{Note that no egocentric video instances are labeled during training.} \YLnote{It may cause confusion as we use labeled ego data for pre-trained models. Shall we remove it?} TN: Yes, agreed. 
Once pre-trained, the video backbone can be directly fine-tuned for a downstream egocentric task.%\cc{, or used in conjunction with the distillation losses to further improve performance.}
% \TNnote{TODO: Reference fig better in text.}
% \YLnote{I meant figure bottom-right: do we want 'Distillation task heads' instead of 'Task distillation heads'?} %TN: I think Task distillation heads is fine. Let me know if you strongly prefer the other! % Okay.
%\KGnote{try to use some of the key notation, like $H$ etc.}
}
\vspace{-5mm}
\label{fig:framework}
\end{figure*}

\section{Ego-Exo Approach}
% \TNnote{Consistency issue? Auxiliary task, aux loss, aux distillation loss, aux ego-task?}
% \YLnote{need addressing the consistency among video, clips and features notations ($x$, $x_t$, $f_m$)}
% \TNnote{each video instance is $v$. $v = {x_1, ... x_N}$ --- these are clip features $(c, t, h, w)$ tensors. $v$ is also $= {f_1 ... f_T}$ --- these are input frames. $x$ is used to refer to a generic clip feature (i.e. any $x_i$).}

% \KGnote{Decide if it is Object-score or Object-Score, etc. for all three.}
% \YLnote{Let's use Ego-Score, Object-Score and Interaction-Map}





% Our Ego-Exo approach aims to learn ego-specific video representations with existing third-person datasets, e.g. Kinetics. The proposed model is expected to learn features that are predictive of some ego-specific clues while still inheriting good video representations for general video understanding. Hence, we introduce a novel Ego-Exo pre-training framework which adds several ego-inspired tasks to embed ego-specific clues into the pre-trained model. 
Our goal is to learn egocentric video representations from third-person video datasets, by discovering and distilling  %. Third-person videos contain 
important cues about hands, objects, and interactions (albeit in a different viewpoint) that are relevant to egocentric activity during pre-training. %, and focusing on these cues helps map features learned for third person video to features that are useful for egocentric video understanding.  \KGnote{if needed could shorten this para a lot and merge into next one.}
% we automatically generate ego-related labels to teach the video model during pre-training.  Those ego-related labels are designed to describe some representative ego properties, like how likely the video is egocentric, what and where are the manipulating objects.
To do this, we automatically assign third-person video instances with various egocentric pseudo-labels that span simple similarity scores %(e.g., how \emph{egocentric-like} is this video?) \YLnote{remove the examples to save space as they will also occur in Sec 3.2.}
to complex spatiotemporal attention maps, %
%(e.g., what are likely spatiotemporal regions for hand-object interactions?),
%and we
and then we introduce auxiliary losses that force our features to be predictive of these pseudo-labels. 
% On one hand, we still keep the action classficiation task with original labels to take advantages of the diverse actions and large-scale videos in third-person datasets.  On the other hand, for the additional auxiliary ego tasks, instead of adding any manually annotated labels for the third-person dataset, ...
On the one hand, our approach retains the benefits of large-scale third-person video and the original action classification task to guide general video feature learning. On the other hand, we steer feature learning towards better egocentric features using automatically generated egocentric labels, as opposed to collecting manually labeled instances.

% In the following, we first detail the proposed three ego-specific labels in Ego-Exo, including Ego-score (Sec~\ref{sec:ego-score}, Object-score (Sec~\ref{sec:object-score} and Interaction-map (Sec~\ref{sec:interaction}). Then, we explain the full pipeline of Ego-Exo approach in Sec~\ref{sec:pipeline}
In the following sections, we first describe the traditional video pretraining framework (Sec~\ref{sec:background}) %general Ego-Exo pre-training framework that 
and how we incorporate our auxiliary loss terms into it (Sec~\ref{sec:pre-training}). Next we describe the three egocentric tasks we use, namely Ego-Score, Object-Score, and Interaction-Map (Sec~\ref{sec:tasks}). Finally, we present our full training and evaluation pipeline in Sec~\ref{sec:pipeline}. % \TNnote{names of tasks?}

%  Specifically, we incorporate the above ego-specific tasks to pre-train the video model on exo dataset, and then fine-tune on pre-trained model to different downstream ego understanding tasks.

%  Intuition: 1) As ego and exo videos intrinsically contains domain gap, we introduce a general ego-score to measure the general egocentricity of a video, which encourage the video representation to discriminate ego and exo videos.
% 2) Most actions in ego videos are manipulating objects~\cite{epic, charades-ego}, so we introduce another two ego-inspired tasks to require the video model to be predictive of manipulatated objects and spatialtemporal hand-object interaction regions.


% \KGnote{spell out more what is the intuition -- we want the video features to inherit the good action understanding from the exo data, but at the same time be predictive of egocentric-specific facets (?)} 
% \KGnote{at the onset, can we say why this is the ``right" list of things to preserve?  at least we can make the intuitive case}
% \YLnote{Good point! Will add the intuition parts.}

%\BOnote{In method, should we first discuss the overall framework, and then discuss each component?}
%\YLnote{Sounds good!}



% \TNnote{1. Framework, 2. Ego tasks, 3. Putting them together}

\subsection{Video model pre-training} \label{sec:background}

% \TNnote{I added some notation just so that it'll be easy to point it out in diagrams. $M^\tau$ is pretty unnecessary Cut if you want.}

% \KGnote{maybe early in approach we should notate all pools of data we are assuming access to / and/or all models?  there is a pool of third-person video labeled by activity (e.g., Kinetics); there is a set of data labeled as being first-person or third-person,...  consider consolidating the assumptions about what we have access to (and will make clear what we \emph{don't} have access to.}

% We augment third-person video model pre-training with auxiliary egocentric loss terms. For this, we build on the standard video pre-training task --- action classification. 

Video models benefit greatly from strong initializations. The standard procedure for training egocentric video models is thus to first pre-train models using large-scale third-person video datasets, and then fine-tune for a specific downstream task.

% regular action recognition background
More formally, we are provided with a large-scale third-person (exocentric) video dataset $\mathcal{V}_{exo}$. In pre-training, each video instance $v \in \mathcal{V}_{exo}$ consists of $T$ frames $\{f_1, ..., f_T\}$ and an associated action label $y^{act}$. These frames are encoded into a series of $N$ spatiotemporal clip features $\{x_1, ..., x_N\}$, where $x_i \in \mathbb{R}^{c \times t \times h \times w}$, using a video encoder \emph{backbone} (e.g., a 3D CNN model). These features are then passed to a classifier \emph{head}, which spatiotemporally pools the feature and uses a linear classifier to generate the predicted action class $\hat{y}^{act}$. % generate the prediction $\hat{y}_a = W^T \mathcal{P}(x) + b$, where $W, b$ are the classifier parameters, and $\mathcal{P}$ is the average-pooling operator.
Predictions are typically generated for each clip and then averaged to generate video-level predictions. The network is trained to minimize the cross entropy loss $\mathbb{L}_{act}(y^{act}, \hat{y}^{act})$. See Fig~\ref{fig:framework} (left panel). 

Once pre-trained, the backbone weights are retained, the head is replaced with a task-specific classifier, and the new network is trained with instances from a target egocentric dataset $\mathcal{V}_{ego}$ to predict egocentric video labels.
% \YLnote{I am thinking if we want to shorten this background paragraph. For example, some notations actually appear once and are not important, like $\mathcal{P}$, $W, b$.}
% Removed

\subsection{Ego-Exo pre-training} \label{sec:pre-training}
% this isn't enough
Third-person pre-training alone results in strong, general-purpose video features.  However, it ignores important egocentric signals %that are useful for downstream egocentric video tasks 
and introduces a domain gap that limits its utility for downstream egocentric tasks. %performance.
We introduce auxiliary egocentric task losses to overcome %account for 
this gap.

% details
Specifically, along with datasets $\mathcal{V}_{exo}$ and $\mathcal{V}_{ego}$, we assume access to off-the-shelf %pre-trained 
video models that address a set of egocentric video understanding tasks. 
For each task $\tau$, the model $M^\tau$ takes as input a video (as either frames or clips) and generates predicted labels $y^\tau$. We use these pre-trained models to associate egocentric \emph{pseudo-labels} to the third-person video instances in $\mathcal{V}_{exo}$.  We stress that the videos in $\mathcal{V}_{exo}$ are \emph{not} manually labeled for any task $\tau$.

We introduce %modify the default pre-training procedure to include 
a task-specific head $H^\tau$ for each task that is trained to approximate these pseudo-labels for each video instance, leading to an auxiliary loss term $\mathbb{L}_{\tau}(H^\tau(v), y^\tau)$. Each head is trained to approximate the response of an egocentric video model when applied to a third-person video instance, and thus can be seen as a knowledge-distillation mechanism %\cite{hinton2015distilling} 
that distills %privileged   % KG don't need to cite again?
% \KGnote{I don't think this needs to be considered ``privileged" since predicted?} % TN: Agreed
information from the egocentric tasks into the video encoder model.
The final pre-training objective is the combination of the action classification loss $\mathbb{L}_{act}$ and each of the auxiliary loss terms $\mathbb{L}_{\tau}$. See Fig~\ref{fig:framework} for our full framework.
% \TNnote{Looks like there are some references to $f_ego$ branches in other sections. Add some text about them here.}

% rationalize choices
Note that these pseudo-labels vary in structure and semantics, ranging from scalar scores (e.g., to characterize how \emph{egocentric-like} a third-person video is), categorical labels (e.g., to identify the manipulated objects in video) and spatiotemporal attention maps (e.g., to characterize hand-object interaction regions). Moreover, these labels are egocentric-specific, but they are \emph{automatically} generated for third-person video instances.  This diverse combination 
%\cc{of target labels and structures} 
leads to robust feature learning for egocentric video, as our experiments will show. 
%\cc{As before,} 
Once pre-trained, we can retain our \emph{enhanced} backbone weights to fine-tune on an egocentric video task using data from $\mathcal{V}_{ego}$.

% teaser
% In the following sections, we describe each of the tasks we use, how we source the models $H_\tau$ and labels $y_\tau$ for video instances, the specific loss term $\mathbb{L}_{\tau}$ used for each task, and their relevance to egocentric feature learning.

\subsection{Auxiliary egocentric tasks}\label{sec:tasks}
Next, we describe each task we use, how we source $M^\tau$ and pseudo-labels $y^\tau$, the %specific 
loss terms $\mathbb{L}_{\tau}$, and their relevance to egocentric feature learning. Note that no egocentric activity labels are used for the task models, and each task model is applied to third-person video instances in $\mathcal{V}_{exo}$.
%---no egocentric video instances are labeled for activities.} 
%\YLnote{I understanding the second sentence explains for aux tasks, but I feel the first and second sentence seem unrelated and it will cause additional confusion as we only use third-person videos for pretraining. Maybe we could just remove it?} %\KGnote{careful, because we use labeled ego data to train ego-classifier} 
%\TN{I'm okay with removing this. This is going to be a pretty sticky point to deal with for reviews too, so I think we should plan on where/how to bring it up, if not here. Remind us about this when we meet next!} \KGnote{I think pointing out they are applied to exo here is useful.  As for the ``no ego labels" what if we qualify by ``in pre-training"?  I feel like keeping this straight may be hard for a reviewer.}
%\YLnote{bring to the meeting}
%\vspace{-4mm}
%\paragraph{Ego-Score: Discriminating ego videos.}

\vspace{-3mm}
%\noindent\textbf{Ego-Score: Discriminating ego videos.}
\paragraph{Ego-Score: Discriminating ego videos.}
% Compared to third-person videos, egocentric videos provide their own exclusive information, \eg a unique viewpoint, reflection on the camera wearer's motions and interactions. For video understanding tasks, good egocentric video representations are desired to be able to discriminate ego videos from third-person videos, thus capturing the underlying egocentric-specific properties. 
%\cc{Egocentric videos offer a unique viewpoint that is strongly tied to the camera wearer's motion and interactions.} 
A good egocentric video representation should be able to capture the underlying differences between first- and third-person videos, to discriminate between the two viewpoints. Based on this motivation, we design
an \textit{Ego-Score} task $\tau^{ego}$ %for each video
to characterize the egocentricity likelihood of the video. 

% Then we introduce the auxiliary task to encourage the pre-trained features to be predictive of the Ego-score. In this way, the learned pre-trained features should be able to tell which videos are mostly or least like egocentric videos. The basis for this procedure is an ego classifier that could discriminate egocentric and third-person videos, thus estimating the Ego-score for each video.
% TN: redundant now

% We train the ego classifier as a binary classifier on the Charades-Ego dataset~\cite{charades-ego}, which contains two sets of egocentric and third-person videos. The reason why we are not take other popular third-person datasets with egocentric videos to construct the training dataset is that the trained ego classifier might cheat easily according to some unrelated clues, including different action sets and scenarios (e.g. popular third-person datasets~\cite{kinetics} contains more sports and outdoor actions while egocentric datasets~\cite{epic,li2018eye} focuses more on interaction objects and indoor scenes). In Charades-Ego, the egocentric and third-person video sets share the same action set, even more having paired videos. Thus, the trained ego classifier is expected to focus more on the critical clues to discriminate egocentric and third-person videos.
For this, we train a binary \emph{ego-classifier} $M^{ego}$ on the Charades-Ego dataset~\cite{charades-ego}, which has both egocentric and third-person videos of indoor %in the indoor domain, of 
activities involving object interactions. % We choose this dataset for its focus on indoor activities involving object interactions, and because the videos from both viewpoints are from the same domain. 
 While the dataset offers paired instances showing the same activity from two views, our method does not use this pairing information or egocentric activity labels. 
%\KGnote{but we do use kinetics activity labels. maybe say ``no egocentric activity labels"?  and if that appears here we could cut that phrase above.} \YLnote{sounds good!}
It uses only the binary labels indicating if a sample is egocentric or exocentric. \YL{Please see Supp.~for more training details and an ablation study about the %of
pairing information.}

% We use a standard 3D CNN (Slow model~\cite{slowfast}) as backbone to train the ego classifier. Then, we perform the trianed ego classifier on the third-person dataset (\eg Kinetics) which is used for pre-training to estimate the Ego-score $y^{ego}$ for each Kinetics video $x$. As the ego classifier is a clip-based network, we sampled several clips among the video and then aggregate them to obtain the video-level Ego-score.
We use this trained classifier to estimate the real-valued pseudo task-labels $y^{ego}$ for each video in our pre-training framework described in Sec~\ref{sec:pre-training}. We sample multiple clips from the same video and average their score to generate a video-level label. % To formalize, let us denote the video as $x = \{x_1, ..., x_N \}$, where $x_n$ is the $n^{th}$ sampled clip. For each clip $x_n$, the score is generated by the predicted logits $z^{ego}_i(x_n)$ from the ego classifier, where $i \in \{0, 1\}$ is the class label. Then we average the per-clip logits and apply a `softmax` layer to produce a probability as Ego-score:
Formally, for a video $v$ with $N$ clips $\{x_1, ..., x_N \}$ we generate scores:
\vspace{-0.5mm}
\begin{equation}
y_i^{ego}(v) = \frac{\exp(\frac{1}{N\beta} \sum_{n} z^{ego}_i(x_n))}{\sum_{j} \exp(\frac{1}{N\beta} \sum_{n}{z^{ego}_j(x_n))}}, \label{eqn:yego}
%\vspace{-1mm}
\end{equation}
where $\beta$ is a scalar temperature parameter, $z^{ego}_i(x_n)$ is the predicted logits from the ego-classifier $M^{ego}$, and $i \in \{0, 1\}$ is the class label. %\TNnote{Simplify this? I don't think we need to write out softmax.} 

% \YLnote{The current implementation is averaging the logits. For KD loss, I think the inputs should be teacher's and student's logits instead of probability, right? That's why I average the logits here.}
 
%\YLnote{Averaging over logits or probability both look fine to me. Do you have any references that we should averaging probability? I am following Disinit~\cite{girdhar2019distinit}, thus averaging over logits.}
% Then, we add a Ego-score prediction branch $f^{ego}$ for the video model as shown in Fig~\ref{fig:framework} and the Ego-score $y^{ego}$ is used as soft targets for training a student network by a knowledge-distillation loss~\cite{hinton2015distilling}:
% KD stuff absorbed in prev section
Third-person videos display various egocentric cues, resulting in a broad distribution of values for Ego-Score, despite sharing the same viewpoint (details in Supp).
This score is used as the soft target in the auxiliary task loss, which we predict using a video classification head $H^{ego}$: %We use a module $H^{ego}$ that spatially pools clip features, and then uses a fully connected layer to predict this score.
\begin{equation}
    \mathbb{L}_{ego}(x) = -\sum_{i} y^{ego}_i(v)\ \log (H^{ego}_i(x)).
\vspace{-4mm}
\end{equation}

% \begin{itemize}
%     \item Train a data-driven ego classifier which is used to discriminate if a video is egocentric or not. Specially, we could conduct the videos from ego datasets as positive samples and videos from third-person datasets as negative samples. 
%     \item Perform the ego classifier on the exo dataset which is used for pre-training. Get \textit{ego-score} for each video using the predicted score from the ego classifier. 
%     \item Use ego-score as the pseudo label during exo dataset pre-training by adding an auxiliary knowledge distillation loss. 
% \end{itemize}

%\vspace{-3mm}
%\vspace{1mm}
%\noindent\textbf{Object-Score: Finding interactive objects.}
\vspace{-2mm}
\paragraph{Object-Score: Finding interactive objects.}
%\TNnote{IMPORTANT: Are these spatiotemporal boxes for hands/objects, or just spatial? I've been saying spatiotemporal everywhere. Doesn't look like from approach text. Need to correct text if so.}
%\YLnote{For object score, we are averaging per-frame score to generate a video-level score. So it's not spatial. But for handobject, it's spatiotemporal.}
%As a unique viewpoint
In egocentric videos, %actions with
interactions with objects are often central, as evident %draw most attentions in egocentric video understanding, which could also be revealed 
in popular egocentric video datasets~\cite{charades-ego,epic,li2018eye}. 
% This motivates us to encourage video representations to be predictive of manipulated objects. %, which could be helpful for egocentric video understanding. 
% Thus, we designate an \textit{Object-Score} task $\tau^{obj}$ for each video to potentially find interactive objects in the video. % and make the video model to be predictive of the Object-Score.
Motivated by this, we designate an \textit{Object-Score} task $\tau^{obj}$ for each video that encourages video representations to be predictive of manipulated objects.

Rather than require %As we do not have 
ground-truth object labels for third-person videos, we propose a simple solution that directly uses an off-the-shelf object recognition model $M^{obj}$ trained on ImageNet~\cite{deng2009imagenet} 
%(\eg a ResNet model~\cite{resnet}) 
to describe objects in the video. Formally, for a video $v$ with frames $\{f_1, ..., f_T\}$ %Similar to the Ego-Score,%
we average the predicted logits from $M^{obj}$ %the image-level recognition model among multiple 
across frames to generate the video-level Object-Score $y^{obj}_i(v)$:  
%\KGnote{CHECK: in sec 3 opening, x is defined as spatiotemporal feature, but here it is a video clip and $x_m$ is a frame?}
\begin{equation}
    y^{obj}_i(v) = \frac{\exp(\frac{1}{T\beta} \sum_{t} z^{obj}_i(f_t))}{\sum_{j} \exp(\frac{1}{T\beta} \sum_{t}{z^{obj}_j(f_t))}}, \label{eqn:yobj}
\end{equation}
%where $f_t$ is the $t^{th}$ frame among $M$ sampled frames in $\mathcal{V}$ and
where $z^{obj}_i(f_t)$ is predicted logits for the $i^{th}$ class from the recognition model, and $\beta$ is the temperature parameter. 

Similar to the Ego-Score, we introduce %We again use 
a knowledge-distillation loss during pre-training to make the video model predictive of the Object-Score using a module $H^{obj}$:
\begin{equation}
    \mathbb{L}_{obj}(x) = -\sum_{i} y^{obj}_i(v) \log H^{obj}_i(x).
\vspace{-3mm}
\end{equation}
% where $f^{obj}(x)$ is the predicted object score. %during pre-training. 

% \KGnote{Why is it $f$ here but $H$ for model for ego score above?}

% \begin{itemize}
%     \item We use an off-the-shelf standard image-level object recognition (e.g. a ResNet model trained on ImageNet~\cite{deng2009imagenet}) to generate object-score.
%     \item Specifically, for each video in the exo dataset, we uniformly sample several frames from each clip and perform the ImageNet model on the sampled frames. Then we average the predicted scores of the multiple frames to obtain the video-level object-score.
%     \item Similar to ego-score, we use object-score as the pseudo label during exo dataset pre-training by adding an auxiliary distillation loss.
% \end{itemize}

% \vspace{-3mm}

\paragraph{Interaction-Map: Discovering hand interaction regions.}
%\noindent\textbf{Interaction-Map: Discovering hand interaction regions.}
The %above
Object-Score attempts to describe the interactive objects. Here we explicitly %further
focus on the spatiotemporal regions of interactions in videos. 
% As shown in~\cite{li2018eye}, with only small regions around the gaze point, \KG{it is possible to recognize a} camera wearer's actions, as her gaze point usually focuses on the interaction region \KG{where hand-object manipulations occur}. 
Prior work shows it is possible to recognize a camera wearer's actions by attending to only a small region around the gaze point~\cite{li2018eye}, as gaze often focuses on hand-object manipulation.
Motivated by this, % This motivates us 
we introduce an \textit{Interaction-Map} task $\tau^{int}$ to learn features that are
%to encourage the pre-trained model to be 
predictive of these important spatiotemporal hand-object interaction regions in videos. 

\begin{figure}[t]% [htbp]
\centering
\includegraphics[width=\columnwidth]{figs/interaction_map1}
\vspace{-7mm}
\caption{\textbf{Interaction-Map construction.} Soft-labels for hand-map and object-map are generated from detected bounding boxes according to Eqn~\ref{eq:bbox}.
}
\vspace{-5mm}
\label{fig:interaction-map}
\end{figure}

We adopt an off-the-shelf hand-object detector~\cite{shan2020understanding} $M^{int}$ to detect hands and interacting objects. %We apply the hand-object detector on the frames of the third-person videos to obtain the bounding boxes for hands and interacting objects. Then, we generate a hand-map and a object-map for each frame, which together compose the Interaction-Map. 
% See Fig~\ref{fig:interaction-map}.
%As Fig~\ref{fig:interaction-map} shows,
% Specifically, we first generate a $k \times k$ hand-map $y^h$ for each frame, where $k$ could be \KGnote{is?} the same as the size of feature map from the last layer of the video backbone. The bounding boxes of the detected hands are projected into the $k \times k$ image score and denoted as $\{(b^h_1, s^h_1),...,(b^h_k, s^h_k)\}$ where $b^h_k$ and $s^h_k$ are the corresponding hand bounding box and score for \KG{the} $j^{th}$ \KG{detected} hand. \KGnote{what is $b$ exactly, a 2d point and scale?} 
For each frame $f_t$ in a video, the hand detector predicts a set of bounding-box coordinates and associated confidence scores $\mathcal{B}^t = \{(b^h, s^h)\}$ for detected hands. These bounding boxes are scaled to $h \times w$---the spatial dimensions of the video clip feature. % For each grid \KG{cell} $(i, j)$ in the hand-map, the score $y^h_{i, j}$  is %related to 
We then generate a $t \times h \times w$ spatiotemporal hand-map $y^{h}$ where the score for each grid-cell $y^{h}_{i, j} (f_t)$ at each time-step is calculated by its overlap with the detected hands at time $t$: %\TNnote{(r,c) --- weird indexing ?}
\begin{align}
\vspace{-1mm}
     y^{h}_{i, j} (f_t) = 
    \begin{cases}
    \max_{k \in \mathcal{B}^t_{i, j}}\{s^h_k\} & \text{if} ~~~~ \mathcal{B}^t_{i, j} \neq \emptyset, \\
    0 & \text{if} ~~~~ \mathcal{B}^t_{i, j} = \emptyset,
    % 0 & \text{if } grid_{i, j} \text{ has no overlapping with all} {b^h_k},
    % s & \text{otherwise}
    \end{cases}  
 %   & \mathcal{B} = \{j~~ |~~ is\_overlap(b^h_k, grid_{i, j}) = True\} 
 %& \KG{ \mathcal{B} = b^h_k \cap grid_{i, j}}
    \label{eq:bbox}
\vspace{-1mm}
\end{align}
where $\mathcal{B}^t_{i, j}$ % = b^h_k \cap grid_{i, j}$} %$is\_overlap(b, grid_{i, j})$
%checks if bounding box $b\TN{_k}$ overlaps with $grid_{i, j}$.
is the set of predicted bounding boxes that overlap with the $(i, j)$-th grid-cell at time $t$. The full hand-map label $y^h$ is formed by concatenating the per-frame labels over time.
We generate the corresponding object-map $y^o$ analogously. See Fig~\ref{fig:interaction-map} for an illustrative example.

%Then, 
We use the hand-map and object-map as the Interaction-Map pseudo-labels for the third-person videos during pre-training. We introduce two Interaction-Map prediction heads, $H^h$ and $H^o$, % after the backbone of the video model %predicted the interaction-map and
% supervised by the binary cross-entropy loss:
to directly predict the $t \times h \times w$ Interaction-Map labels from clip features using a 3D convolution head:
\begin{equation}
\vspace{-1mm}
\begin{split}
    % \mathbb{L}_{int}(x) = - \sum_{t} \left[
    %         \sum_{0 \leq i, j < k} y^{h}_{i, j}(x_t) \log H^{h}_{i, j}(x_t)\\
    %         + \sum_{0 \leq i, j < k} y^{o}_{i, j}(x_t) \log H^{o}_{i, j}(x_t) 
    %         \right] ,
    \mathbb{L}_{int}(x) = - \sum_{i, j} \Bigg( \Bigg.
    \sum_{k} y^{h}(f_k) \log [H^{h}(x)]_k \\
    + y^{o}(f_k) \log [H^{o}(x)]_k 
    \Bigg. \Bigg)_{i, j},
\end{split} \label{eq:int-map}
\vspace{-3mm}
\end{equation}
where $f_k$ is $k$-th frame from training clip $x$, and $H^{h}(x)$ and $H^{o}(x)$ are the predicted hand-map and object-map scores. %\TNnote{Looks so messy. Can we make this equation easier to parse?}
% \KGnote{
%as above - the first one uses $H$ but the others use $f$. 
% also check the notation consistency of $x$, $x_t$, $x_m$ and feature volume $x$.}
%$y^h(f_t)$, $y^o(f_t)$
%The reason why

\cc{We predict Interaction-Maps instead of directly predicting bounding boxes % coordinates
via standard detection networks~\cite{ren2015faster} for two reasons. 
First, detection architectures are not directly compatible with standard video %model
backbones---they %, and work well only on higher resolution inputs. 
typically utilize specialized backbones %with large receptive field
and work well only with %feed with 
high resolution inputs. %for accurate localization, which is not directly compatible with standard video model backbones.
% \TNnote{True?} \YLnote{I think it's still possible to use video backbone, so I tried to make our argument weaker.} %models require larger input size and some specific designs on the backbone while we still want to keep the original backbone of the video model. 
Second, predicting scores on 
a feature map %adding the constraint loss on the feature map reflects our 
is more aligned with our ultimate goal to improve the feature representation for egocentric video tasks, rather than train a precise detection model.  }
%\KGnote{also isn't the model we are using object-agnostic (vs. ~\cite{ren2015faster} where we'd have to enumerate the objects to detect? and the hands part is also critical?}
% ^ YL is making an argument for why we're predicting heatmaps instead of bbox coordinates, not hands/objects vs. general object classes.

% \begin{itemize}
%     \item We use an off-the-shelf hand-object detector~\cite{shan2020understanding} to detect hands and interacting objects. Specifically, we perform the hand-oject detector for the frames from the videos in the exo dataset to obtain the bounding boxes for hands and interacting objects. 
%     \item As Fig~\ref{} shows, we first generate a $k \times k$ hand-map for each frame. Each grid in the hand-map is either $0$ if the grid has no overlaps with hand boxes or the corresponding box score if the grid has overlaps with any hand boxes. Similarly, we could generate the object-map.
%     \item We use the hand-map and object-map as the pseudo labels of interaction-map for exo videos during pre-training. We add an interaction-map prediction head to the specific layers in the model backbone to predict the interaction-map and supervised by the binary cross-entropy loss.
% \end{itemize}

\subsection{Ego-Exo training and evaluation}\label{sec:pipeline}
The three proposed ego-specific auxiliary tasks are %could be
combined together during the pre-training procedure to construct the final training loss:
\vspace{-1mm}
\begin{equation}
%\vspace{-5mm}
\vspace{-1mm}
\begin{split}
     \mathbb{L}(x) = \mathbb{L}_{act}(x) &  + w_{ego} * \mathbb{L}_{ego}(x) \\
            +  w_{obj} & * \mathbb{L}_{obj}(x) + w_{int} * \mathbb{L}_{int}(x),
\end{split} \label{eqn:loss}
%\vspace{-5mm}
\end{equation} 
%\vspace{-1mm}
where $\mathbb{L}_{act}$ is the standard cross-entropy loss for third-person action recognition, and $w_{ego}$, $w_{obj}$ and $w_{int}$ are the corresponding loss weights for the three auxiliary tasks, selected via cross-validation %independently for
on downstream tasks. %\KGnote{set with cross validation?  with what labeled data - the specific downstream task's data?}
%\YLnote{Yes, it's set with cross-validation on the downstream validation set of charades-ego and epic-55 dataset. I am thinking how about explaining it on the experiments section, like Implementation details?} 
% TN: Yes. Explain all this in implementation details.

% \YL{Note that all third-person videos contribute to both the action recognition loss $\mathbb{L}_{act}$ and the auxiliary losses. For %the
% videos without hand-object regions or \TN{salient} %big
% interactive objects, our egocentric tasks %could 
% still generates valid pseudo-labels as we utilize soft targets in the distillation loss. Meanwhile, the soft targets have higher entropy, thus providing much more information during pre-training than hard targets or directly ignoring negative samples. 
%}
Note that third-person video instances without hand-object interactions or salient interactive objects still contribute to the auxiliary loss terms, and are not ignored. Our distillation models %aim  to 
approximate the \emph{responses} of the pre-trained egocentric models as soft-targets instead of hard labels, offering valuable information about perceived egocentric cues, whether positive or negative for the actual label. %\YL{Meanwhile, the soft targets have higher entropy, thus providing much more information during pre-training than hard targets or directly ignoring negative samples.} 
% \TNnote{I don't follow the entropy point?}
% \YLnote{I am trying to say soft targets are better than hard targest or ignoring nagative samples, as soft distributions have higher entropy, thus having more information}
% TN: I don't think we have to spell this part out. I just added soft-targets in brackets.

% \KGnote{discussion: comment on how it is not the case that every third-person video will have hand-object regions or big objects etc., but that's ok because... conceptually about the method.}\YLnote{add the above paragraph}

Training with our auxiliary losses results in features that are more suitable for downstream egocentric tasks, but it does not modify the network architecture itself. Consequently, after pre-training, our model can be directly used as a drop-in replacement for traditional video encoders, and it can be applied to various egocentric video tasks. 
% As we have no requirements for the video network and no modifications on the backbone structure, generally the proposed Ego-Exo could be applied to different video networks and utilized as the initialization weights for different egocentric video tasks.  
% \KGnote{should we briefly allude to how many / which backbones are studied in expts?} 
% \YLnote{For backbones, we actually only take two types, Slow model and SlowFast. Should we emphasize this?}
% \TNnote{No. Just reference in the exp section I think.}




% \BOnote{Do we use the auxiliary losses in fine-tuning as well? }
% \YLnote{Yes, plan to have the ablation study on Sec 4.2 and Table~\ref{tb:add_loss_to_ego}. How about describing it in the the ablation study?}



% \begin{itemize}
% \item pre-train the video model on exo dataset by adding the one or multiple above proposed auxiliary losses.
% \item Take the backbone of the pre-trained model as initalization and fine-tune the whole video model in the ego datasets.  \KGnote{are all our results with full fine tuning, or did we have any luck with freezing and just training last layer?}
% \end{itemize}





==> Ego-Exo_CVPR21 (ArXiv)_4:14:2021/sections/related.tex <==
\begin{section}{Related Work}

% \KGnote{decide if we are saying pre-trained or pre-trained throughout.} 
% \YLnote{Let's fix it to pre-trained and spatiotemporal if there is no preference?}
% \YLnote{Use pre-trained everywhere}

\paragraph{Egocentric video understanding}
% \begin{itemize}
% \item Different ego datasets are collected to facilitate egocentric video understanding domains, like EGTEA, charades-EGO, Epic-Kitchen. The scale is still not comparable to popular third-person datasets. \KGnote{should we be concrete here? and also try not to overly emphasize ``labeled dataset size" as the sole shortcoming that we overcome...since that's just a matter of time and money.}
% \item Different ego tasks, like Recognition, anticipation, gaze detection, egocentric video summarization, etc.
% \item Plenty of works have been proposed to improve the video representations for egocentric video understanding, like structured video representation~\cite{ego-topo,others}, multi-modal modeling~\cite{epic-fusion}. 
% \item In contrast, our model focusing on the exo-dataset pre-training stage, which provides a general exo-pre-trained models which should be able to adopted by different methods for different ego datasets and tasks.
% \end{itemize}
The unique viewpoint in egocentric video presents interesting research challenges including action recognition and anticipation~\cite{zhou2015temporal,furnari2020rolling,rhinehart2017first,abu2018will}, daily life summary generation~\cite{lee2015predicting,yonetani2016visual}, inferring body pose~\cite{jiang2017seeing,ng2020you2me}, and estimating gaze~\cite{li2013learning,huang2018predicting}. Several egocentric video datasets have been created to support these challenges~\cite{epic,li2018eye,pirsiavash2012detecting,charades-ego}. Model architectures proposed for these tasks include multi-stream networks~\cite{ma2016going,li2018eye,epic-fusion,wang2020makes}, recurrent networks~\cite{furnari2019would,furnari2020rolling,sudhakaran2019lsta}, 3D conv nets~\cite{pirri2019anticipation,lu2019learning} and spatially grounded topological graph models~\cite{ego-topo}.  % \TNnote{YL, check if all these cites are \emph{representative} enough} 

These architectures vary significantly, but all use video encoders that are similarly pre-trained with third-person video datasets, despite being applied to egocentric video tasks. In contrast, we introduce key egocentric losses during \emph{exocentric video} pre-training that bridge the domain gap when applied to downstream egocentric video tasks. 
% \TNnote{Too vague?} 

\vspace{-3mm}
\paragraph{Joint first/third person video understanding} % fix subsection name
% \begin{itemize}
% \item Something about multiple views (not necessarily egocentric) [Optional]

% \item Prior work has focused on learning \emph{domain-invariant} representations for first and third person video using embedding learning methods. This has been applied to action recognition~\cite{soran2014action,sigurdsson2018actor,ardeshir2018exocentric}, video summarization with limited labeled egocentric data~\cite{ho2018summarizing}, cross-view image retrieval~\cite{fan2017identifying} and person segmentation~\cite{xu2018joint}. 

% \item \cite{yu2019see} augments embedding learning approaches with an attention module that encourages similar spatiotemporal attention masks between first-person and third-person videos, resulting in improved gaze prediction, summarization and segmentation. \KGnote{if we itemize this one out, seems to need a stronger contrast statement against ours.}% Can be merged above.
% % \item \cite{ho2018summarizing} encodes video using two backbones --- a shared one, and a domain-specific one. They use a triplet loss for matching shared features, and minimize dot product between domain specific ones to make them different.

% \item Image generation methods~\cite{elfeki2018third,regmi2018cross,regmi2019bridging,liu2020exocentric} use generative adversarial frameworks to synthesize the egocentric viewpoint from a third person view (or vice-versa).  \KGnote{are they doing this for sake of better recognition / learning?} TN: No, just pretty images
% \item Prior work uses the egocentric video as a supplementary modality to improve person identification and tracking when combined with top-view surveillance footage ~\cite{ardeshir2016ego2top, ardeshir2018integrating,ardeshir2016egoreid}, pose identification and tracking~\cite{yang2018ego}.
% % \cite{ardeshir2016ego2top} devices a graph-based matching method to associate egocentric video of people in a scene to videos taken from a top-view camera, in order to improve person identification.

% \item Contrast: The above methods usually require datasets with paired third-person and first-person videos, which affects the generalization of the method and is limited in relatively small datests. \KGnote{which ones do not require paired data?  it will be stronger if we divide them up so don't have to say ``usually require"}  Our method is general to adopt a general large-scale third-person dataset for pre-training without any requirement for ego dataets.
% \end{itemize}

Several strategies have been proposed to address the domain gap between first and third person video. Prior work learns \emph{viewpoint-invariant} representations using embedding learning methods, and applies them to action recognition~\cite{soran2014action,sigurdsson2018actor,ardeshir2018exocentric}, video summarization~\cite{ho2018summarizing}, image retrieval~\cite{fan2017identifying}, person segmentation~\cite{xu2018joint}, and attention-driven gaze prediction~\cite{yu2019see}. 
Image generation methods~\cite{elfeki2018third,regmi2018cross,regmi2019bridging,liu2020exocentric} use generative adversarial frameworks to synthesize one viewpoint from the other.  Viewpoint invariance has also been treated as a \emph{domain adaptation} task in prior work, adapting third-person video models for overhead drone-footage~\cite{choi2020unsupervised}.
Other methods use egocentric video as a modality to supplement top-view footage to improve identification and tracking models~\cite{ardeshir2016ego2top, ardeshir2018integrating,ardeshir2016egoreid,yang2018ego}. 
%\KGnote{reg img generation: are those papers doing anything with video / recognition?  or just the generation?}
% TN: Just generation (they measure Inception score, SSIM, etc.)

The above methods require \emph{paired} datasets that are either simultaneously recorded or that share the same labels for instances across viewpoints. In contrast, our method leverages only third-person video datasets, but is augmented with pseudo-labels (derived from first-person models) to learn egocentric video representations, thus circumventing both the need for first-person video during pre-training and the need for paired labeled data.


% \paragraph{Domain adaptation for video} % Need to look for more
% \begin{itemize}
% \item Prior work learns domain-invariant features for video via adversarial domain adaptation methods. 
% \item \cite{choi2020unsupervised} transfers features from third-person video for action recognition with drone footage.
% \item \cite{kae2020image} performs domain adaptation from webly-supervised images and videos to a target video dataset. 
% \item \cite{yao2019adversarial} treats different temporal distributions of actions as \emph{domains} and learns classifiers that are robust to changes in this distribution (e.g. always seeing ``running'' before ``kicking'' in training vs. arbitrary orders in testing). % Doesn't fit well here

% \item Contrast: Unlike prior work, we consider the two viewpoints --- egocentric vs. third-person --- as distinct domains and devise specialized auxiliary losses to achieve domain adaptation, rather than the general feature invariance considered in prior work. % weak
% Meanwhile, different domain adaptation method needs access to data in the specific target domain during training, our work focuses on the pre-training stage without requirement to access any samples in the target ego domain.

% % \KGnote{should we have a generic domain adaptation baseline?}
% % YLnote{as discussed, will have one in the result comparison.}
% \end{itemize}

\vspace{-3mm}
\paragraph{Knowledge distillation for video} 
% \begin{itemize}
% \item General: Knowledge distillation (KD) has been used to compress models~\cite{hinton2015distilling,mullapudi2019online,chen2017learning}, to incorporate privileged information from alternate tasks~\cite{lopez2015unifying}. % Lots more here

% \item In videos, KD has been used to incorporate information from alternate modalities like audio~\cite{gao2020listen,aytar2016soundnet}, depth and flow~\cite{gupta2016cross,stroud2020d3d} or a combination of modalities~\cite{luo2018graph}.

% \item It has also been used to incorporate privileged information such as object-level information~\cite{pan2020spatio}.

% \item \cite{girdhar2019distinit} uses an ImageNet pre-trained model to assign weak labels to video instances in order to train video-level models. Compared to \cite{girdhar2019distinit}, we use pre-trained models that are relevant to the egocentric domain (hand-object interaction), along with the video-level labels rather than in place of them. % make stronger later


% \item In contrast to the above, we use object-interaction information from an alternate viewpoint (egocentric) rather than an alternate modality, to perform distillation. 

% \TNnote{Is this relevant? \cite{camporese2020knowledge}}
% \BOnote{Use distillation during pre-training and fine-tuning \cite{chen2020big}.} 

% \end{itemize}

In knowledge distillation (KD), one network is trained to reproduce the outputs of another~\cite{hinton2015distilling}.  Distillation %has been proposed to compress
serves to compress 
models~\cite{hinton2015distilling,mullapudi2019online,chen2017learning} or incorporate privileged information from alternate tasks~\cite{lopez2015unifying}. In videos, KD can incorporate information from alternate modalities like audio~\cite{gao2020listen,aytar2016soundnet}, depth and flow~\cite{gupta2016cross,stroud2020d3d}, or a combination
%of modalities
~\cite{luo2018graph}, 
and %to incorporate privileged 
object-level information~\cite{pan2020spatio}.
In the context of self-supervised learning, prior work assigns weak image labels to video instances as supervision for video-level models~\cite{girdhar2019distinit}. In contrast, we use inferred weak labels 
that are relevant to the egocentric domain, %(namely egocentricity and hand-object interaction labels)
and we use them alongside third-person video labels, rather than in place of them during pre-training.

% \TNnote{Is this relevant? \cite{camporese2020knowledge}} No

% \BOnote{Use distillation during pre-training and fine-tuning \cite{chen2020big}. We can just add the reference in approach when we discuss using distillation for fine-tuning.} \YLnote{As it's image-level semi-supervised paper, what's the best place if we want to explicitly talk about it?} 


% \paragraph{Object/Hand attention/detection?} % name better
% \begin{itemize}
% \item Prior work has improved egocentric video understanding models by incorporating specialized features for the egocentric setting~\cite{li2015delving,ma2016going}.
% \item Attention mechanisms derived from gaze and motor attention~\cite{mathe2012dynamic,li2018eye,liu2019forecasting}
% \item Active object detections~\cite{baradel2018object,dessalene2020egocentric,}...
% \item Prior work on human-object interaction understanding has focused on detecting hands in contact~\cite{tekin2019h,shan2020understanding,kapidis2019egocentric}. 
% \item Contrast: We are also interested in hand-object interactions, but unlike prior work we do not train models on labeled egocentric video datasets in order to detect these. Instead, we use hand-object interactions as an auxiliary loss in \emph{third-person video} models to steer feature learning towards egocentric relevant features.
% \item Lots more relevant citations to add here if we want to focus on this ...
% \end{itemize}

% \paragraph{Multi-task cross domain stuff...} % absorbed in object/hand

\vspace{-3mm}
\paragraph{Egocentric cues in video understanding models}
Egocentric video offers several unique cues that have been leveraged to improve video understanding models~\cite{li2015delving,ma2016going}. These include attention mechanisms from gaze and motor attention~\cite{mathe2012dynamic,li2018eye,liu2019forecasting}, active object detection~\cite{antonino-next-active,baradel2018object,dessalene2020egocentric,wang2020symbiotic}, and hands in contact~\cite{tekin2019h,shan2020understanding,kapidis2019egocentric}.
We are also interested in such important egocentric cues, but unlike prior work we do not train models on labeled egocentric video datasets %in order 
to detect them. Instead, we embed labels predicted for these cues as auxiliary losses in \emph{third-person video} models to steer feature learning towards egocentric relevant features. %\TNnote{More here?}
Unlike any of these prior methods, our goal is to leverage third-person video to pre-train first-person video models.

% \BOnote{Could we have fewer numbers of clusters of related work?}
% TN: Squashed to 4
\end{section}
